Marginalizable Density Models

Probability density models based on deep networks have achieved remarkable success in modeling complex high-dimensional datasets. However, unlike kernel density estimators, modern neural models do not yield marginals or conditionals in closed form, as these quantities require the evaluation of seldom tractable integrals. In this work, we present the Marginalizable Density Model Approximator (MDMA), a novel deep network architecture which provides closed form expressions for the probabilities, marginals and conditionals of any subset of the variables. The MDMA learns deep scalar representations for each individual variable and combines them via learned hierarchical tensor decompositions into a tractable yet expressive CDF, from which marginals and conditional densities are easily obtained. We illustrate the advantage of exact marginalizability in several tasks that are out of reach of previous deep network-based density estimation models, such as estimating mutual information between arbitrary subsets of variables, inferring causality by testing for conditional independence, and inference with missing data without the need for data imputation, outperforming state-of-the-art models on these tasks. The model also allows for parallelized sampling with only a logarithmic dependence of the time complexity on the number of variables.

==> Marginalizable Density Models (4)/arxiv/ack.tex <==
\section*{Acknowledgements}

The work of DG is supported by a Swartz fellowship. 
The work of AP is supported by the Simons Foundation, the DARPA NESD program, NSF NeuroNex Award DBI1707398 and The Gatsby Charitable Foundation.

==> Marginalizable Density Models (4)/arxiv/design_details.tex <==
%!TEX root = ../MDM_arxiv.tex

\section{Additional design details} \label{app:design_details}


\subsection{Univariate marginal parameterization} 
\label{app:univariate_marginal_param}

We parameterize the univariate marginal CDF $\varphi(x)$ for some scalar $x \in \mathbb{R}$ using a simple feed-forward network following \cite{balle2018variational}. Recall from section \Cref{sec:theory} that we model the univariate CDFs as functions
\begin{align*}
     \varphi(x) = \mbox{sigmoid} \circ L_{l} \circ \sigma_{l-1} \circ L_{l-1} \circ \sigma_{l-2} \cdots \circ \sigma_1 \circ L_1 \circ \sigma_0 \circ L_0(x),
\end{align*}
where $L_i \colon \R^{n_{i}} \to \R^{n_{i+l}}$ is the affine map $L_i(x) = W_i x + b_i$ for an $n_{i+1} \times n_{i}$ weight matrix $W_i$ with \emph{nonnegative} elements and an $n_{i+1} \times 1$ bias vector $b_i$, with $n_{l+1} = n_0 = 1$ and $n_i = r$ for $i \in [l]$. This is a slightly more general form than the one in \Cref{sec:theory} since we allow the nonlinearities to depend on the layer. For the nonlinearities, we use 
% \begin{equation*}
% \begin{aligned} & \alpha^{0}(x) & = & \,\, x,\\
%  & {\alpha}^{\ell}(x) & = & \,\, g^{\ell}({W}^{\ell}{\alpha}^{\ell-1}(x)+{b}^{\ell}),\\
%  & F(x) & = & \,\, \sigma({W}^{L_{u}}{\alpha}^{L_{u}-1}(x)+{b}^{L_{u}}),
% \end{aligned}
% \end{equation*}
% where 
\begin{equation*}
   \sigma_i({x})={x}+{a_i}\odot\tanh({x})
\end{equation*}
for some vector $a_i \in \mathbb{R}^{n_{i+1}}$ with elements constrained to lie in $[-1, 1]$ (the lower bound on $a_i$ is necessary to ensure that $\sigma_i$ are invertible, but the upper bound is not strictly required). This constraint, as well as the non-negativity constraint on the $W_i$, is enforced by setting ${W}_i=\mathrm{softplus}(\tilde{{W}}_i,10),{a_i}=\tanh(\tilde{{a}}_i)$ in terms of some $\tilde{{W}}_{i}\in\mathbb{R}^{n_{i+1}\times n_{i}},\tilde{{a}}_{i}\in\mathbb{R}^{n_{i+1}}$. The softplus function is $\mathrm{softplus}(x,\beta)=\frac{1}{\beta}\log(1+\exp(\beta x))$ and is a smooth, invertible approximation of the ReLU. We typically use small values for $l,r$ in the experiments (see \Cref{app:exp_details}).  
% and $\sigma$ is the sigmoid function. $L_u$ is the depth of the network, and ${W}^{\ell}\in\mathbb{R}_{+}^{r_{\ell}\times r_{\ell-1}},{a}^{\ell}\in\mathbb{R}_{+}^{r_{\ell}},{b}^{\ell}\in\mathbb{R}^{r_{\ell}}$ are trainable parameters. Non-negativity of the parameters is ensured by a parameterization ${W}^{\ell}=\mathrm{softplus}(\tilde{{W}}^{\ell}),{a}^{\ell}=\tanh(\tilde{{a}}^{\ell})$ in terms of some $\tilde{{W}}^{\ell}\in\mathbb{R}^{r_{\ell}\times r_{\ell-1}},\tilde{{a}}^{\ell}\in\mathbb{R}^{r_{\ell}}$.  
% The widths of the layers are given by $r_\ell$, and we require $r_0=r_{L_u}=1$. The non-negativity constraints are required to ensure that the derivative w.r.t. the input is non-negative, which combined with the bound on the range induced by the sigmoid ensures that this is a valid PDF. We typically choose $L_u=2$ and $r_1=r_2=r_3\equiv r = 3$ in our experiments.  

 \subsection{Adaptive variable coupling}

One degree of freedom in constructing a HT decomposition is the choice of partitions of subsets of the variables at every layer over which the products are taken.
This imposes a form of weight-sharing, and it will be natural to share weights between variables that are highly correlated.
As a simple example, let $d=4$ and consider two different HT decompositions
\begin{align*}
   F(x_{1},x_{2},x_{3},x_{4})=\underset{i_{1},i_{2},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{1},1}^{1}\lambda_{k,i_{2},2}^{1}\varphi_{i_{1},1}(x_{1})\varphi_{i_{1},2}(x_{2})\varphi_{i_{2},3}(x_{3})\varphi_{i_{2},4}(x_{4}),\\
    \widetilde{F}(x_{1},x_{2},x_{3},x_{4})=\underset{i_{1},i_{2},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{1},1}^{1}\lambda_{k,i_{2},2}^{1}\varphi_{i_{1},1}(x_{1})\varphi_{i_{1},3}(x_{3})\varphi_{i_{2},2}(x_{2})\varphi_{i_{2},4}(x_{4}),
\end{align*}
obtained by coupling $X_1$ in the first layer respectively with $X_2$ and $X_3$.
The univariate marginals for $X_1$, $X_2$ and $X_3$ can then be written as
\begin{align*}
       F(x_{1})=\underset{i_{1},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{1},1}^{1}\varphi_{i_{1},1}(x_{1}),\   F(x_{2})=\underset{i_{1},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{1},1}^{1}\varphi_{i_{1},2}(x_{2}),\  F(x_{3})=\underset{i_{2},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{2},2}^{1}\varphi_{i_{2},3}(x_{3}), \\
       \widetilde{F}(x_{1})=\underset{i_{1},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{1},1}^{1}\varphi_{i_{1},1}(x_{1}),\ \widetilde{F}(x_{2})=\underset{i_{2},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{2},2}^{1}\varphi_{i_{2},2}(x_{2}),\ \widetilde{F}(x_{3})=\underset{i_{1},k}{\sum}\lambda_{k}^{2}\lambda_{k,i_{1},1}^{1}\varphi_{i_{1},3}(x_{3}).
\end{align*}
Assume that the variables $X_1$ and $X_2$ are identical. 
In $F$, both of their univariate marginals depend in an identical way on the tensor parameters.
In $\widetilde{F}$ however, additional parameters are required to represent them.
Hence $F$ is a more parsimonious representation of the join distribution.
If $X_1$ and $X_3$ are identical instead, then the converse holds and $\widetilde{F}$ is the more parsimonious representation.
This property extends to any higher-dimensional (e.g., bivariate) marginals.

In data with spatial or temporal structure (e.g. if the variables are image pixels) there is a natural way to couple variables based on locality. When this is not present, we can adaptively construct the couplings based on the correlations in the data using a simple greedy algorithm. After constructing an empirical covariance matrix from a minibatch of data, we couple the two variables that are most correlated and have not yet been paired. We repeat this until we couple all the groups of variables. Then we "coarse-grain" by averaging over blocks of the covariance matrix arranged according to the generated coupling and repeat the process, this time coupling subsets of variables. We find that this coupling scheme improves performance compared to naive coupling that does not take correlations into account. 

\subsection{Initialization}

As in the univariate case, the non-negativity constraint of the HT tensor parameters $\lambda_{k,k',j}^{i}$ is enforced by defining $\lambda_{k,k',j}^{i}=\mathrm{softplus}\left(\tilde{\lambda}_{k,k',j}^{i},20\right)$ for some $\tilde{\lambda}_{k,k',j}^{i}\in\mathbb{R}$. 

As is standard, we initialize independently the elements of the univariate PDF weights $\tilde{W}_i$ as zero-mean gaussians with variance $1/n_{\mathrm{fan_in}}$, the $\tilde{a}_i$ as standard gaussians and the $b_i$ as 0. The initialization of the HT parameters is $\tilde{\lambda}_{k,k',j}^{i} = m * \delta_{k,k'}$ for $1\leq i\leq p-1$. This initialization is chosen so that after applying the softplus the matrix $\lambda_{\cdot,\cdot,j}^{i}$ is close to an identity at initialization, which we have found facilitates training compared to using a random initialization. Benefits of such ``orthogonal'' initialization schemes have also been shown for deep convolutional networks \cite{xiao2018dynamical, Blumenfeld2020-lu}. The final layer $\tilde{\lambda}_{k}^{p}$ are initialized as zero mean gaussians with variance $0.3/m$.  

\subsection{From HT to MERA}

The choice of the diagonal HT decomposition \cref{eq:HT} is convenient, yet there is a wealth of other tensor decompositions that can be explored. Here we highlight one such decomposition that generalizes the diagonal HT and could potentially lead to more expressive models. It is based on \cite{Giovannetti2008-pk}. 

Let $F^{\mathrm{M},1}\colon \R^d \to \R^{m \times d}$ be a matrix-valued function such that $F^{\mathrm{M},1}_{i,j}(\bm x) = F^{\mathrm{HT},1}_{i,j}(\bm x) = \varphi_{i,j}(x_j)$.
For $l \in \{2, \dots, \log_2 d\}$, define the matrix-value functions $F^{\mathrm{M},1}\colon \R^d \to \R^{m \times d/2^{l-1}}$ recursively by 
\begin{align*}
F^{\mathrm{M},l}_{i,j}(\bm x)  &= 
%  \sum\limits_{k,k'=1}^{m,m'}  \lambda_{k,i,j}^{l-1} \chi_{k',k,i,j}^{l-1}\varphi_{k,2j-1}^{\mathrm{M},l-1}(\bm x)\varphi_{k + k' - 1,2j}^{\mathrm{M},l-1}(\bm x) \\
  \sum\limits_{k}^{m}  \lambda_{k,i,j}^{l-1} \{ \chi_{1,k,i,j}^{l-1}\varphi_{k,2j-1}^{\mathrm{M},l-1}(\bm x)\varphi_{k,2j}^{\mathrm{M},l-1}(\bm x) +  \chi_{2,k,i,j}^{l-1}\varphi_{k,2j-1}^{\mathrm{M},l-1}(\bm x)\varphi_{k + 1,2j}^{\mathrm{M},l-1}(\bm x)\}
\end{align*}
with $k+1 \equiv 1$ when $k = m$, $\lambda^{l}$ as in \eqref{eq:HT_recurs}, and $\chi^{l}$ a $2 \times m \times m \times d/2^{l}$ tensor with nonegative elements satisfying $\chi_{1,k,i,j}^{l}+\chi_{2,k,i,j}^{l} = 1$.
% \begin{align*}
%     \chi_{i_1, i_2, i, j} \chi_{i_3, i_4, i, j} &= \delta_{i_1, i_3} \delta_{i_2, i_4} \\
%      \chi_{i, j, i_1, i_2} \chi_{i, j, i_3, i_4} &= \delta_{i_1, i_3} \delta_{i_2, i_4} \\
%      \lambda_{i_1, i, j} \lambda_{i_2, i, j} &= \delta_{i_1, i_2} \\
%      [\lambda \chi]_{i_1, i_2, i_3, i_4, i_5} &= \lambda_{i_1, j, i_4} \chi_{i_2, i_3, j, i_5}\\
%      [\chi \lambda]_{i_1, i_2, i_3, i_4, i_5} &= \chi_{i_1, i_2, i_4, j} \lambda_{j, i_3, i_5}
% \end{align*}
The MERA parametrization of a distribution can then be written as
\begin{align*}
 F_{\mathrm{M}}(\bm x) &= \sum\limits_{k=1}^m a_{k} \varphi_{k,1}^{\mathrm{M},\log_{2}d}(\bm x)\varphi_{k,2}^{\mathrm{M},\log_{2}d}(\bm x),
\end{align*}
with $a \in \mathbb{R}^m$% with $a$ an $m \times 1$ vector as in \eqref{eq:CP}.
Since the conditions on $\lambda^{l}$ and $\chi^{l}$ imply $\sum\limits_{k=1}^m\lambda_{k,i,j}^{l}(\chi_{1,k,i,j}^{l}+\chi_{2,k,i,j}^{l}) = 1$, this parametrization clearly results in a valid CDF.
Note that $\chi_{1,k,i,j}^{l}+\chi_{2,k,i,j}^{l} = 1$ leads to $\chi^{l}$ having only $m \times m \times d/2^{l}$ free parameters.
% {\color{red}TODO: relate the $\lambda^l$, $\chi^l$ and $a$ tensors to $A$.}
For $d=4$, we have
\begin{align*}
  F_{\mathrm{M}}(\bm x) 
 %  \sum\limits_{k_1=1}^m a_{k_1} \varphi_{k_1,2}^{\mathrm{M},2}(\bm x)\varphi_{k_1,2}^{\mathrm{M},2}(\bm x) \\
  &= \sum\limits_{k_1,k_2,k_2'=1}^m a_{k_1} \lambda_{k_2,k_1,1}^{1} \lambda_{k_2',k_1,2}^{1}\sum\limits_{i_1,i_2=1}^2  \chi_{i_1,k_2,k_1,1}^{1}\chi_{i_2,k_2',k_1,2}^{1}  \\
  &\phantom{ = \sum\limits_{k_1,k_2,k_2',k_3,k_3',k_3'',k_3'''=1}^m } \times \varphi_{k_2,1}^{\mathrm{M},1}(\bm x)\varphi_{k_2 + i_1 - 1,2}^{\mathrm{M},1}(\bm x)\varphi_{k_2',3}^{\mathrm{M},1}(\bm x)\varphi_{k_2' + i_2 - 1,4}^{\mathrm{M},1}(\bm x).
  \end{align*}

==> Marginalizable Density Models (4)/arxiv/discussion.tex <==
%!TEX root = ../MDN_neurips.tex

\section{Discussion}
\label{sec:discussion}
MDMAs offer the ability to obtain, from a single model, closed form probabilities, marginals and conditionals for any subset of the variables. These properties enable one to straightforwardly use the model to solve a diverse array of problems, of which we have demonstrated only a few: mutual information estimation between arbitrary subsets of variables, inference with missing values, and conditional independence testing targeted at multivariate causal discovery. 
In addition to these, MDMA's marginalization property can be used for anomaly detection with missing values~\cite{dietterich2018anomaly}. We have shown that MDMA can fit data with missing values without requiring imputation, yet if one is interested in data imputation for downstream tasks, the ability to sample from arbitrary conditional distributions means that MDMA can be used for imputation as well. 

Additionally, in some application areas (e.g., financial risk management), powerful models exist for the univariate distributions, and marginal distributions are then glued together using copulas~\cite{mcneil2015quantitative}.
However, popular copula estimators suffer from the same drawbacks as modern neural network density estimators with regard to marginalization and conditioning. Using MDMA for copula estimation (say by replacing the kernel density estimator by MDMA in the formulation of \cite{Geenens2017-tg}), one can then obtain copula estimators that do not suffer from these deficiencies. 

The main shortcoming of MDMA is the linearity in the combination of the products of univariate CDFs which appears to limit the expressivity of the model. The study of tensor decompositions is an active area of research, and novel constructions, ideally adapted specifically for this task, could lead to improvements in this regard despite the linear structure. 

==> Marginalizable Density Models (4)/arxiv/exp_UCI.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Density estimation on real data}

We trained MDMA/nMDMA and the non-marginalizable variant described in \Cref{sec:nmdma} on a number of standard density estimation benchmarks from the UCI repository,\footnote{http://archive.ics.uci.edu/ml/datasets.php} following the pre-processing described in \cite{papamakarios2017masked}. 
\Cref{tab:UCI} compares test log likelihoods of 
MDMA/nMDMA with several other neural density models.  
We find the performance of MDMA on the lower-dimensional datasets  comparable to state-of-the-art models, while for higher-dimensional datasets it appears to overfit. nMDMA achieves state-of-the-art performance on the POWER ($d=6$) dataset, but at the cost of losing the ability to marginalize or condition over subsets of the variables. The width of MDMA was chosen based on a grid search over $\{500, 1000, 2000, 3000, 4000\}$ for each dataset, and the marginal CDF parameters by a search over $\left\{ \left(l=2,w=3\right),\left(l=4,w=5\right)\right\}$. All models were trained using ADAM with learning rate $0.01$, and results for MDMA and nMDMA are averaged over $3$ runs.  
Additional experimental details are provided in \Cref{app:exp_details}. 

\begin{table}[]
\caption{\textbf{General density estimation.} Test log likelihood for density estimation on UCI datasets. The comparison results are reproduced from \cite{bigdeli2020learning}.
}
\begin{tabular}{lcccc}
\toprule
Model  &   {\small POWER} {\footnotesize [d=6]}  &  {\small GAS} {\footnotesize [d=11]}           & {\small HEPMASS} {\footnotesize [d=21]}   & {\footnotesize MINIBOONE } {\footnotesize [d=43]}        \\ 
\hline
Kingma et al. 2018   \cite{kingma2018}      & $0.17 \pm .01$ & $8.15 \pm .4$            & $-18.92 \pm .08$         & $-11.35 \pm .07$          \\
Grathwohl et al. 2019     \cite{grathwohl2018ffjord}      & $0.46 \pm .01$ & $8.59 \pm .12$           & $-14.92 \pm .08$         & $-10.43 \pm .04$          \\
Huang et al. 2018         \cite{huang2018neural}          & $0.62 \pm .01$ & $11.96 \pm .33$          & $-15.08 \pm .4$          & $-8.86 \pm .15$           \\
Oliva et al. 2018         \cite{oliva2018transformation}  & $0.60 \pm .01$ & $\mathbf{12.06} \pm .02$ & $-13.78 \pm .02$         & $-11.01 \pm .48$          \\
De Cao et al. 2019 \cite{de2020block}                                         & $0.61 \pm .01$ & $\mathbf{12.06} \pm .09$ & $-14.71 \pm .38$         & $-8.95 \pm .07$           \\
Bigdeli et al. 2020 \cite{bigdeli2020learning}                                                  & $0.97 \pm .01$ & $9.73 \pm 1.14$          & $\mathbf{-11.3} \pm .16$ & $\mathbf{-6.94} \pm 1.81$ \\ \hline
MDMA       &       $0.57 \pm .01$                                   &       $8.92 \pm 0.11$         &      $-20.8 \pm .06$                                 &      $-29.0 \pm .06$                     \\
nMDMA                                            &           $\mathbf{1.78} \pm .12$         &   $8.43 \pm .04$                       &         $-18.0 \pm 0.91$                 &  $-18.6 \pm .47$    
\\

\bottomrule
\end{tabular}
\label{tab:UCI}
\vspace{-.1in}
\end{table}

==> Marginalizable Density Models (4)/arxiv/exp_admv.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Anomaly detection with missing values}

Let $X_1, \dots, X_N$ be an i.i.d. sample with an observation $X_j \in \R^d$ which being either \emph{normal} or an \emph{anomaly}, that is semantically distinctive but without a label to be classified as such.
Loosely speaking, an anomaly detector is a function $s \colon \R^d \to \R$ assigning an anomaly score to every value is $\R^d$.
For instance, given a density estimator $\widehat{f}$, a natural detector is $s(x) = - \log \widehat{f}(x)$ for $x\in \R^d$, that is observations with low density are potentially anomalous.

Additionally, let $M_j, \dots, M_N$ be a vector with $M_j \in \{0,1\}^d$ such that $M_{ji} = 1$ indicates that $X_{ji}$ is missing, and denote by $X_{j(0)}$ and $X_{j(1)}$ respectively the vectors of observed and missing components of $X_j$.
Assume that some values are missing at random or completely at random \citep[MAR or MCAR, see e.g., ][Section 1.3]{little2019}.
In this setup, we can ignore the missingness mechanism and the negative log-likelihood on the observed features, namely $- \sum_{j=1}^N \log f(X_{j(0)})$, is sufficient for inference.

Accounting for potential missingness, the optimal detector is then the conditional expectation of $s$ given the available information, that is
\begin{align*}
    s_{OPT}(x_{(0)}) = \int s(x) \widehat{f}(x_{(1)}|x_{(0)}) dx_{(1)}.
\end{align*}
If the integral is infeasible, an alternative is to use maximum a posteriori imputation (MAP) and compute
\begin{align*}
    s_{MAP}(x_{(0)}) = s(x_{(0)},\widehat{x}_{(1)}),\quad
    \widehat{x}_{(1)} = \mbox{argmax}_{x_{(1)}} \widehat{f}(x_{(1)}|x_{(0)}).
\end{align*}



==> Marginalizable Density Models (4)/arxiv/exp_causal.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Conditional independence testing and causal discovery}

Randomized control trials \cite{Fisher1936} remain the golden standard for causal discovery.
Nonetheless, experiments or interventions are seldom doable, e.g. due to  financial or ethical considerations.
Alternatively, observational data can help uncovering causal relationships \cite{Spirtes2000, Maathuis2015}.
In this context, a class of popular methods targeted at recovering the full causal graph, like PC or FCI \citep{Spirtes2000,strobl2019}, rely on conditional independence (CI) tests.
Letting $X$, $Y$ and $Z$ be random variables, the CI of $X$ and $Y$ given $Z$, denoted $X \independent Y \mid Z$, means that given $Z$, no information about $X$ (or $Y$) can be gained by knowing the value of $Y$ (or $X$).
And testing $H_0\colon X \independent Y \mid Z$ against $H_1\colon X \not \independent Y \mid Z$ is a problem tackled in econometrics \citep{su2007consistent,su2008nonparametric}, statistics \citep{huang2010testing,shah2020hardness}, and machine learning \citep{zhang2011,petersen2021testing}.

Following \citep{petersen2021testing}, denote $U_1 = F(X\mid Z)$ and $U_2 = F(Y\mid Z)$.
It is clear that $H_0$ implies $U_1 \independent U_2$, although the converse does not hold \citep[see e.g.,][]{spanhel2016partial}.
Nonetheless, $U_1 \not \independent U_2$ implies $H_1$, so a test based on the independence between $U_1$ and $U_2$ can still have power.
While the test from \citep{petersen2021testing} is based on estimating the conditional CDFs through quantile regression, we proceed similarly, albeit using the MDMA as a plugin for the conditional distributions.
Our approach is especially appealing in the context of causal discovery, where algorithms require computing many CI tests to create the graph's skeleton.
Instead of having to regress for every test, MDMA estimates the full joint distribution, and its lower dimensional conditionals are then used for the CI tests.

In \Cref{tab:CD}, we present results on inferring the structure of causal graphs using the PC algorithm \cite{Spirtes2000,kalisch2007estimating,sun2007kernel,tillman2009nonlinear,harris2013pc}.
As a benchmark, we use the vanilla (i.e., Gaussian) CI test, and compare it to the PC algorithm obtained with the CI test from \citep{petersen2021testing}, albeit using the MDMA for the conditional distributions.
Synthetic random directed acyclic graphs (DAGs) along with sigmoidal or polynomial mechanisms linking parents to children are sampled using~\cite{JMLR:v21:19-187}.
Each dataset is $d=10$ dimensional and contains 20,000 observations.
We also compare the two algorithms on data from a protein signaling network with $d=11$ \cite{sachs2005causal} for which the ground truth causality graph is known.
Performance is assessed based on the structural Hamming distance (SHD)~\cite{Tsamardinos2006}, that is the $L^1$ norm of the difference between learned adjacency matrices and the truth, as well as a variant of this metric for directed graphs SHD(D) which also accounts for the direction of the edges.
\Cref{tab:CD} shows averages over 8 runs for each setting.
In all cases, MDMA outperforms the vanilla PC in terms of both metrics.
For the synthetic data, we note the large standard deviations, due in part to the fact that we sample randomly from the space of DAG structures, which has cardinality super-exponential in $d$.
An example of the inferred graphs is presented in \Cref{app:additional_exps}.

\begin{table}[]
\caption{\textbf{MDMA for causal discovery.} Conditional densities from a trained MDMA model can be used for causal discovery by allowing to test for conditional independence between variables. Both on synthetic DAG data and real data from a protein signaling network, MDMA infers the graph structure more accurately than a competing method based on quantile regression \cite{petersen2021testing}. The metrics are the structural Hamming distance for the directed (SHD(D)) and undirected (SHD) graph. \label{tab:CD} }
\begin{tabular}{lcccccc}
\toprule
Model & \multicolumn{2}{c}{Sigmoidal DAG, d=10} &  \multicolumn{2}{c}{Polynomial DAG, d=10} & \multicolumn{2}{c}{Sachs \cite{sachs2005causal}, d=11} 
\\ \hline
      & SHD(D)                  & SHD              & SHD(D)                    & SHD                & SHD(D)            & SHD        \\
Gaussian    & $18.6 \pm 3.0$        & $15.6 \pm 2.7$       & $19.8 \pm 4.1$         & $18.9 \pm 4.2$         & 32             & 27             \\
MDMA        & $\mathbf{15.6} \pm 6.1$        & $\mathbf{12.8} \pm 5.2$       & $\mathbf{17.9} \pm 5.3$         & $\mathbf{15.0} \pm 4.5$         & $\mathbf{30.3} \pm 1.8$ & $\mathbf{25.8} \pm 0.7$
\\
\bottomrule
\end{tabular}
\end{table}
% \citep{su2007consistent,su2008nonparametric,huang2010testing,zhang2011,shah2020hardness,petersen2021testing}

% For evaluation we use the structural hamming distance (SHD) as 
% proposed in \citep{Tsamardinos2006} (adding, removing or reversing an edge) 
% necessary to 
% transform one graph to the another and the structural intervention distance 
% (SID), as in \citep{Peters2015}, which is considered to
% be appropriate for quantifying the correct order among variables, by estimating 
% the causal effects they entail.

==> Marginalizable Density Models (4)/arxiv/exp_demv.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Density estimation with missing values} \label{sec:demv}


Dealing with missing values in multivariate data is a classical challenge in statistics that has been studied for decades~\cite{little2019}.
The standard solution is the application of a data imputation procedure (i.e., ``filling in the blanks''), 
which requires making structural assumptions. 
In some cases, this is natural, as for the matrix completion problem under a low-rank assumption~\cite{candes2009exact, candes2010matrix}, where the imputed values are the main object of interest.
But the artifacts introduced by data imputation~\cite{beretta2016nearest}
are generally a price that one must 
unwillingly pay in order to perform statistical inference in models that require fully-observed data points.
Two popular, generic techniques for imputation are MICE~\cite{buuren2010mice} and $k$-NN imputation~\cite{troyanskaya2001missing}.
The former imputes missing values by iteratively regressing each missing variable against the remaining variables, while the latter uses averages over the non-missing values at $k$-nearest datapoints.

More formally, let $X \in \mathbb{R}^{d}$ be distributed according to some density $p$ with parameters $\theta$,  let $X_{(0)}, X_{(1)}$ be the non-missing and missing entries of $X$ respectively, and $M\in\{0,1\}^{d}$ a vector indicating the missing entries. 
In the missing-at-random setting (i.e. $M$ is independent of $X_{(1)}$), 
likelihood-based inference using the full likelihood of the model is equivalent to inference using the marginal likelihood~\cite{little2019} $L(X_{(0)}|\theta)=\int p(X|\theta)dX_{(1)}$.
Standard neural network-based density estimators 
must resort to data imputation because
of the impossibility of computing this marginal likelihood.
MDMA however can directly maximize the marginal likelihood for any pattern of missing data at the same (actually slightly cheaper) computational cost as maximizing the full likelihood, without introducing any bias or variance due to imputation. 


As a demonstration of this capability, we consider the UCI POWER and GAS datasets, following the same pre-processing as \cite{papamakarios2017masked}. We construct a dataset with missing values by setting each entry in the dataset to be missing independently with a fixed probability . We compare MDMA to BNAF~\cite{de2020block}, a neural density model which achieves state-of-the-art results on a number of density estimation benchmarks including GAS. We train MDMA directly on the log marginal likelihood of the missing data, and BNAF by first performing data imputation using MICE \cite{buuren2010mice} and then training using the full log likelihood with the imputed data. The validation loss is the log marginal likelihood for MDMA and the log likelihood of the imputed validation set for BNAF. The test set is left unchanged for both models and does not contain any missing values. We train BNAF using the settings specified in \cite{de2020block} that led to the best performance ($2$ layers and $40d$ hidden units where $d$ is the dimensionality of the dataset). The results are shown in \Cref{fig:missing_data}. 
\begin{figure}
\vspace{-.2in}
  \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/missing_data_power.pdf}
  \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/missing_data_gas.pdf}
  \end{subfigure}
    \caption{\textbf{Density estimation with missing data} Test NLL on two density estimation benchmarks, varying the proportion of entries in each data matrix that are designated missing and not used for fitting. We compare MDMA which can fit marginal densities directly with BNAF which achieves state-of-the-art results on the POWER dataset, after performing data imputation using MICE. As the proportion of missing data increases, MDMA outperforms BNAF.}
    \label{fig:missing_data}
\end{figure}
We find that, as the probability of missingness increases, MDMA significantly outperforms BNAF on both datasets.
Note that, while the proportion of missing values might seem extreme, it is not uncommon in some applications (e.g., proteomics data).
We also trained BNAF using $k$-NN imputation \cite{troyanskaya2001missing}, finding that performance was worse than MICE imputation for all values of $\alpha$.
A comparison of the two methods is provided in \Cref{app:additional_exps}. 

==> Marginalizable Density Models (4)/arxiv/exp_mie.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Mutual information estimation}
Given a multivariate probability distribution over some variables $X=(X_1 \dots ,X_d)$, estimating the mutual information 
\begin{equation}
    I(Y;Z)=\int dp_{X}(x)\log\left(\frac{p_{X}(x)}{p_{Y}(y)p_{Z}(z)}\right),
    \label{eq:MI}
\end{equation}
where $Y,Z$ are random vectors defined by disjoint subsets of the $X_i$, requires evaluating $p_{Y}, p_{Z}$ which are marginal densities of $X$. Typically, $Y$ and $Z$ must be fixed in advance, yet in some cases it is beneficial to be able to flexibly compute mutual information between any two subsets of variables. Estimating both $I(Y,Z)$ and $I(Y',Z')$ may be highly inefficient, e.g. if $Y$ and $Y'$ are highly overlapping subsets of $X$. 
Using MDMA however, we can fit a single model for the joint distribution
and easily estimate the mutual information between \textit{any} subset of variables by simply marginalizing over the remaining variables to obtain the required marginal densities. 
Thus a Monte Carlo estimate of (\ref{eq:MI}) can be obtained by evaluating the marginal densities at the points that make up the training set. 
\Cref{fig:MI_est} presents an example of this method, showing the accuracy of the estimates.
\begin{SCfigure}
    \centering
    \includegraphics[height=1.8in]{figs/MI_estimation.pdf}
    \caption{\textbf{Mutual information estimation between subsets of a random vector.}
    We fitted a single MDMA model to samples from a zero-mean $d=16$ Gaussian, with covariance $\Sigma_{ij}=\delta_{ij}+(1-\delta_{ij})(i+j-2)/(5d)$. 
    Monte Carlo estimates of the mutual information~(\ref{eq:MI}) between 
     $(X_1, \dots, X_k)$ and $(X_{k+1}, \dots, X_d)$ for any $k=1,\dots, d-1$ are easily obtained and match closely the exact values.       For each $k$ we average over 5 repetitions of drawing the dataset and fitting. 
    % After fitting a multivariate Gaussian density, the mutual information between different disjoint subsets of the variables is estimated without requiring any additional fitting, showing good agreement with the ground truth values.
    }
    \label{fig:MI_est}
    \vspace{-.5in}
\end{SCfigure}


% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=4cm}}]{figure}[\FBwidth]
% {\caption{\textbf{Simultaneous mutual information estimation between subsets of a random vector.} After fitting a multivariate Gaussian density, the mutual information between different disjoint subsets of the variables is estimated without requiring any additional fitting, showing good agreement with the ground truth values.}\label{fig:MI_est}}
% {\includegraphics[height=2in]{figs/MI_estimation.pdf}}
% \end{figure}

==> Marginalizable Density Models (4)/arxiv/exp_toy.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Toy density estimation}
\newcommand\subfigwidth{.24\textwidth}

\begin{figure}[h]
  \centering
  \renewcommand{\tabcolsep}{1pt}
  \begin{tabular}[c]{cccc}
\begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data.pdf}
      \label{fig:caeob}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data_2d_1_2.pdf}
      \label{fig:ceoac}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data_2d_1_3.pdf}
      \label{fig:ceose}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data_2d_2_3.pdf}
      \label{fig:ceod}
    \end{subfigure}
    \\[-.1in]
       \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_model_samples_3d.pdf}
      \label{fig:ceob}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_marg_1_2.pdf}
      \label{fig:ceoc}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_marg_1_3.pdf}
      \label{fig:ceoe}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_marg_2_3.pdf}
      \label{fig:cdfeod}
    \end{subfigure}
    \\[-.1in]
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=2.5cm, width=\textwidth]{figs/3d_spirals_1d_marg.pdf}
      \label{fig:caeob}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_cond_0.5.pdf}
      \label{fig:ceoac}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_cond_0.pdf}
      \label{fig:ceose}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_cond_-0.5.pdf}
      \label{fig:ceod}
    \end{subfigure}
  \end{tabular}    
  \caption{\textbf{Density estimation with closed-form marginals and conditionals.} \textit{Top Row:} Samples from the model after fitting a three-dimensional density, and plots of two-dimensional marginal densities learned by the model.
  \textit{Middle Row:} Samples from the training set, and marginal histograms of training data. \textit{Bottom Row:} \textit{Left:} one-dimensional marginals learned by the model compared to marginal histograms of the training data. \textit{Right:} Conditional densities learned by the model. All the marginal and conditional densities can also be sampled from efficiently (not shown).}
  \label{fig:ceo}
\end{figure}




==> Marginalizable Density Models (4)/arxiv/exp_toy_checkerboard.tex <==
%!TEX root = ../MDN_neurips.tex

\begin{figure}[h]
  \centering
  \renewcommand{\tabcolsep}{1pt}
  \begin{tikzpicture}
    \node {\begin{tabular}[c]{cccc}
\begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_data.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_data_2d_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_data_2d_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_data_2d_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in]
       \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_model_samples_3d.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_marg_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_marg_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_marg_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in]
    \begin{subfigure}[c]{\subfigwidth}
    \vspace{.05in}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_1d_marg.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_cond_0.5.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_cond_0.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_cond_-0.5.pdf}
      \label{}
    \end{subfigure}
  \end{tabular}};
    \draw[black,thick,] (-7,2.3) rectangle (7,6.3);
      \node[text width=3cm] at (0.6,6) 
    {Training data};
\end{tikzpicture}
  \caption{\textbf{Density estimation with closed-form marginals and conditionals.}
  \textit{Top Row:} Samples from a 3D density, and 2D marginal histograms. \textit{Middle Row:} Samples from MDMA after fitting the density, and plots of the learned 2D marginals.
  \textit{Bottom Row:} \textit{Left:} learned 1D  marginals compared to 1D marginal histograms of the training data. \textit{Right:} Learned conditional densities.}
  \label{fig:checkerboard}
\end{figure}

==> Marginalizable Density Models (4)/arxiv/exp_toy_combined.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Toy density estimation}
We start by considering  3D augmentations of three popular 2D toy probability distributions 
introduced in~\cite{grathwohl2018ffjord}: two spirals, a ring of  8 Gaussians and a checkerboard pattern. These distributions allow to explore the ability of density models
to capture challenging multimodalities and discontinuities~\cite{de2020block, huang2018neural}.
The results, presented in~\Cref{fig:toy_de}, show that MDMA captures all marginal densities with high accuracy, and samples from the learned model appear indistinguishable from the training data. 
% We evaluate MDMA on a number of low-dimensional toy density estimation tasks, inspired by tasks commonly used in other works on neural-network based density estimators \cite{de2020block, huang2018neural}. Other methods fit two-dimensional datasets, yet we construct three-dimensional versions of these datasets in order to exhibit the ability of MDMA to obtain closed-form marginal and conditional densities. We consider datasets of two spirals, 8 gaussians and a checkerboard pattern, since these are highly multimodal and are thus challenging tasks in low dimensions. We present detailed results for the two spiral dataset in \Cref{fig:2spirals}, with the marginal densities evaluated on a grid. 
% In this same figure we present examples of the marginal densities for the 8 gaussian and checkerboard tasks, with additional results on these tasks presented in \Cref{app:additional_exps}. For all tasks, we find that MDMA captures all marginal densities with high accuracy, and samples from the model appear  indistinguishable from the training data. 
\begin{figure}[h]
  \centering
  \renewcommand{\tabcolsep}{1pt}
  \begin{tikzpicture}
    \node {\begin{tabular}[c]{cccc}
\begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_model_samples_3d.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in]
       \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_0.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_0.5.pdf}
      \label{}
    \end{subfigure}
        \\[-.1in] % --------
    \begin{subfigure}[c]{\subfigwidth}
    \vspace{.05in}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_data_title.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_marg_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_data_title.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_marg_1_2.pdf}
      \label{}
    \end{subfigure}
  \end{tabular}};
    % \draw[black,thick,] (-7,4.2) rectangle (7,8.3);
    %   \node[text width=3cm] at (0.6,8) 
    % {Training data};
        \draw[black,thick,] (-7,2.3) rectangle (3.43,5.8);
      \node[text width=3cm] at (-1,6) 
    {Training data};
\end{tikzpicture}
\vspace{-.3in}
  \caption{\textbf{Density estimation with closed-form marginals and conditionals.} 
  \textit{First Row:} Panels~1,2: Empirical histograms of training data. Panel 3: Samples from the training data. Panel 4: Samples from the trained MDMA model.
  \textit{Second Row:} Panels 1,2: The marginal density learned by MDMA plotted on a grid. Panels 3,4: Conditional densities learned by MDMA plotted on a grid. 
   \textit{Third Row:} Results on additional datasets: Panels 1,2: Training data and learned marginal density for a 3D checkerboard dataset. Panels 3,4: Similarly for a 3D mixture of Gaussians.
   }
  \label{fig:toy_de}
\end{figure}

==> Marginalizable Density Models (4)/arxiv/exp_toy_gaussians.tex <==
%!TEX root = ../MDN_neurips.tex

\begin{figure}[h]
  \centering
  \renewcommand{\tabcolsep}{1pt}
  \begin{tikzpicture}
    \node {\begin{tabular}[c]{cccc}
\begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_data.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_data_2d_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_data_2d_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_data_2d_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in]
       \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_model_samples_3d.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_marg_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_marg_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_marg_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in]
    \begin{subfigure}[c]{\subfigwidth}
    \vspace{.05in}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_1d_marg.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_cond_0.5.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_cond_0.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_cond_-0.5.pdf}
      \label{}
    \end{subfigure}
  \end{tabular}};
    \draw[black,thick,] (-7,2.3) rectangle (7,6.3);
      \node[text width=3cm] at (0.6,6) 
    {Training data};
\end{tikzpicture}
  \caption{\textbf{Density estimation with closed-form marginals and conditionals.}
  \textit{Top Row:} Samples from a 3D  density, and 2D marginal histograms. \textit{Middle Row:} Samples from MDMA after fitting the density, and plots of the learned 2D  marginal.
  \textit{Bottom Row:} \textit{Left:} learned 1D  marginals compared to 1D marginal histograms of the training data. \textit{Right:} Learned conditional densities.}
  \label{fig:8gaussians}
\end{figure}

==> Marginalizable Density Models (4)/arxiv/exp_toy_spirals.tex <==
%!TEX root = ../MDN_neurips.tex

\begin{figure}[h]
  \centering
  \renewcommand{\tabcolsep}{1pt}
  \begin{tikzpicture}
    \node {\begin{tabular}[c]{cccc}
\begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in]
       \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_model_samples_3d.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in] % --------
    \begin{subfigure}[c]{\subfigwidth}
    \vspace{.05in}
      \includegraphics[width=\textwidth]{figs/3d_spirals_1d_marg.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_0.5.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_0.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_-0.5.pdf}
      \label{}
    \end{subfigure}
    %     \\[-.1in] % --------
    % \begin{subfigure}[c]{\subfigwidth}
    % \vspace{.05in}
    %   \includegraphics[width=\textwidth]{figs/3d_checkerboard_data.pdf}
    %   \label{}
    % \end{subfigure}&
    % \begin{subfigure}[c]{\subfigwidth}
    %   \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_marg_1_2.pdf}
    %   \label{}
    % \end{subfigure}&
    % \begin{subfigure}[c]{\subfigwidth}
    %   \includegraphics[width=\textwidth]{figs/3d_gaussians_data.pdf}
    %   \label{}
    % \end{subfigure}&
    % \begin{subfigure}[c]{\subfigwidth}
    %   \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_marg_1_2.pdf}
    %   \label{}
    % \end{subfigure}
  \end{tabular}};
    % \draw[black,thick,] (-7,4.2) rectangle (7,8.3);
    %   \node[text width=3cm] at (0.6,8) 
    % {Training data};
        \draw[black,thick,] (-7,2.3) rectangle (7,6.3);
      \node[text width=3cm] at (0.6,6) 
    {Training data};
\end{tikzpicture}
  \caption{\textbf{Density estimation with closed-form marginals and conditionals.} 
  \textit{First Row:} Samples from the training set, and marginal histograms of training data.
  \textit{Second Row:} Samples from the model after fitting a three-dimensional density, \dg{clarify} and plots of two-dimensional marginal densities learned by the model.
   \textit{Third Row:} \textit{Left:} one-dimensional marginals learned by the model compared to marginal histograms of the training data. \textit{Right:} Conditional densities learned by the model. All the marginal and conditional densities can also be sampled from efficiently.
  \textit{Fourth Row:} Results on additional datasets: \textit{Left:} Training data and learned marginal density for a 3D checkerboard dataset. \textit{Right:} Training data and learned marginal density for a 3D mixture of Gaussians.
   }
  \label{fig:2spirals}
\end{figure}

==> Marginalizable Density Models (4)/arxiv/header.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
 \hypersetup{
     colorlinks=true,
     linkcolor=blue,
     filecolor=blue,
     citecolor = red,      
     urlcolor=cyan,
     }
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{sidecap}

\sidecaptionvpos{figure}{t}

\usepackage{mathtools} % amsmath with fixes and additions
% \usepackage{siunitx} % for proper typesetting of numbers and units
%!TEX root = ../MDN_neurips.tex

\usepackage{booktabs} % commands to create good-looking tables
\usepackage{tikz} % nice language for creating drawings and diagrams
\usetikzlibrary{calc,positioning} 
\usepackage{amsfonts}
\usepackage{cleveref}
\usepackage{bm}
\newcommand\subfigwidth{.24\textwidth}
\usepackage{tabu}
% \usepackage{algorithm, algorithmic}
\usepackage[ruled,vlined]{algorithm2e}
\SetKw{KwBy}{by}
\usepackage{caption}
\usepackage{subcaption}

\crefname{equation}{}{}

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\dg}[1]{{\bf \color{blue} Dar: #1}}
\usepackage[compact]{titlesec}
%\titlespacing{\section}{0pt}{0pt}{0pt}

\newcommand{\eq}{\begin{equation*}}
\newcommand{\en}{\end{equation*}}
\newcommand{\eqa}{\begin{eqnarray*}}
\newcommand{\ena}{\end{eqnarray*}}
\newcommand{\eqn}{\begin{equation}}
\newcommand{\enn}{\end{equation}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\eqan}{\begin{eqnarray}}
\newcommand{\enan}{\end{eqnarray}}
\newcommand{\vp}{\varpropto}
\newcommand{\nn}{\nonumber}
\newcommand{\tab}{\hspace*{1em}}

\newcommand{\J}{ {\bf J} }
\newcommand{\M}{ {\bf M} }
\newcommand{\X}{ {\bf X} }
\newcommand{\V}{ {\bf V} }
\newcommand{\B}{ {\bf B} }
\newcommand{\q}{ {\bf q} }
\newcommand{\s}{ {\bf s} }

\newcommand{\cc}{ {\bf c} }
\newcommand{\bu}{ {\bf u} }
\newcommand{\bfa}{ {\bf a} }
\newcommand{\bb}{ {\bf b} }
\newcommand{\xx}{ {\bf x} }

\newcommand{\E}{{\mathrm{E}}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\eP}{{\mathbb{P}_n}}
\newcommand{\eG}{{\mathbb{G}_n}}
\newcommand{\Fcal}{{\mathcal F}}
\newcommand{\Gcal}{{\mathcal G}}
\newcommand{\Acal}{{\mathcal A}}
\newcommand{\Ccal}{{\mathcal C}}
\newcommand{\Rcal}{{\mathcal R}}
\newcommand{\Xcal}{{\mathcal X}}
\newcommand{\Ical}{{\mathcal I}}
\newcommand{\varphid}{{\dot \varphi}}

\usepackage{dsfont}
\newcommand{\Ind}{\mathds{1}}

\newcommand{\ubar}[1]{\text{\b{$#1$}}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

% theorem environments -------------------------
\usepackage{amsthm}
%\newtheoremstyle{new}{12pt}{12pt}{\itshape}{}{\bfseries}{.}{1em}{}
%\theoremstyle{new}
%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}

==> Marginalizable Density Models (4)/arxiv/intro.tex <==
%!TEX root = ../MDN_neurips.tex

\section{Introduction}\label{sec:intro}

Estimating the joint probability density of a set of random variables is a fundamental task in statistics and machine learning that has witnessed much progress in recent years.
While traditional estimators such as histograms~\cite{scott1979optimal,lugosi1996consistency} and kernel-based methods~\cite{Rosenblatt,parzen1962estimation} have appealing theoretical properties and typically perform well in low dimensions, they become computationally impractical above 5-10 dimensions.
Conversely, recent density models based on neural networks~\cite{kingma2018,huang2018neural,oliva2018transformation,grathwohl2018ffjord,de2020block,bigdeli2020learning} scale efficiently with the number of random variables, but lack a crucial feature available to traditional methods: the ability to compute probabilities, marginalize over subsets of variables, and evaluate conditionals. These tasks require integrals of the estimated density, 
which are intractable for modern neural density models.  
Thus, while such operations are central 
to many applications (e.g., inference with missing data, testing for conditional (in)dependence, or performing do-calculus~\cite{pearl_book}), approaches based on neural networks require estimating separate models 
whenever marginals or conditionals are needed.  

Alternatively, one could model the cumulative distribution function (CDF), making computing probabilities and marginalization straightforward. But evaluating the density requires taking $d$ derivatives of the CDF, which incurs an exponential cost in $d$ for a generic computational graph.
This observation has made direct CDF modeling traditionally challenging~\cite{chilinski2020neural}.

In this work, we present the \emph{marginalizable density model approximator} (MDMA), a novel deep network architecture preserving most of the expressive power of neural models for density estimation, while  providing closed form expressions for the probabilities, marginals and conditionals of any subset of the variables.
In a nutshell, the MDMA learns many deep 
scalar representations for each individual variable 
and combines them using hierarchical tensor decompositions \cite{hackbusch2012tensor,cichocki2016tensor} into a tractable multivariate CDF that can be fitted using stochastic gradient descent.
%While tensor decompositions are not new idea in modern machine learning, this paper is the first, to the best of our knowledge, to leverage it for density estimation.
Additionally, sampling from MDMA can be parallelized along the input dimension, resulting in 
a very low space complexity and a time complexity that scales only logarithmically with the number of variables in the problem (as opposed to linearly in naive autoregressive sampling, see below in \Cref{sec:related}). 
% \dg{should we mention other benefits of having a CDF model i.e. anomaly detection?}

As could be expected, the architectural choices that allow for easy marginalization take  a minor toll  in terms of performance. Indeed, while competitive, our model admittedly does not beat  state-of-the-art models in out-of-sample log-likelihood of 
high-dimensional datasets. On the other hand, it does 
beat those same models in a task for which the latter are ill-prepared: learning densities from data containing missing values, a
common setting in some application areas such as genomics~\cite{li2009genotype, marchini2010genotype}. 
While our model is able to deal optimally with missing values by evaluating, for every data point,  the marginal likelihood over its non-missing values, other models must resort to data
imputation. Consequently, we significantly outperform state-of-the-art neural density estimators trained 
using a number of common data imputation strategies. We also show MDMA can be used to test for conditional independence, which is useful for discovering the causal structure in graphs, a task on which it outperforms existing methods, and that it enables estimation of mutual information between arbitrary subsets of variables after fitting a single model. Additionally, we prove that the model class is a universal approximator over the space of absolutely continuous multivariate distributions. 


The structure of this paper is as follows. In \Cref{sec:related} we 
review related works. In \Cref{sec:marginalizable_models} we
present our new model and its theoretical properties.
We present our experimental results in~\Cref{sec:experiments}, and 
conclude in~\Cref{sec:discussion}. 




==> Marginalizable Density Models (4)/arxiv/litterature.tex <==
%!TEX root = ../MDN_neurips.tex

\section{Related work}
\label{sec:related}

Modern approaches to non-parametric density estimation, 
based on normalizing flows~\cite{kingma2018,huang2018neural,oliva2018transformation,grathwohl2018ffjord,de2020block,bigdeli2020learning} (see~\cite{kobyzev2020normalizing,papamakarios2021normalizing} for recent reviews), model expressive yet invertible functions that transforms a simple (usually uniform or Gaussian) density to the target density.
Nonetheless, as previously mentioned, such architectures 
lead to intractable derived quantities such as probabilities, marginals and/or conditional distributions.

Moreover, many normalizing flow models rely on an autoregressive construction, 
which makes the cost of generating samples scale linearly with the dimension.
This can be circumvented using inverse autoregressive flows~\cite{kingma2016improving}, but in this dual case a linear cost 
is incurred instead in density evaluations and hence in training. Another solution is training a feed-forward network using the outputs of a trained autoregressive model~\cite{oord2018parallel}. With MDMA, fast inference and sampling is achieved without requiring this distillation procedure. 




Tensor decompositions~\cite{hackbusch2012tensor,cichocki2016tensor}, 
which are exploited in this work, have been used in various applications 
of signal processing, machine learning, computer vision, and more~\cite{vasilescu2002multilinear,cichocki2009nonnegative,anandkumar2014tensor,papalexakis2016tensors,sidiropoulos2017tensor}.
Recently, such decompositions have been used to speed-up or reduce the number of parameters in existing deep architectures~\cite{lebedev2014speeding,tai2015convolutional,novikov2015tensorizing,kim2015compression,yang2016deep,chen2018sharing}.
In addition to their practical appeal, 
tensor methods have been widely studied to understand the success of deep neural networks \cite{cohen2016expressive,haeffele2015global,janzamin2015generalization,janzamin2015beating,sharir2017expressive}



% {\color{red}
% \begin{itemize}
%     \item related work (generative modeling, density estimation) 
%     \item why they can't do everything - we can discuss what existing methods do and don't do along the lines of section 2 of https://arxiv.org/pdf/1804.00779.pdf
%     \item missing values and composite likelihood (in the discussion maybe?)
% \end{itemize}
% }


==> Marginalizable Density Models (4)/arxiv/mdma.tex <==
%!TEX root = ../MDN_neurips.tex

\section{Marginalizable Density Models}
\label{sec:marginalizable_models}

\subsection{Notation}
In the following, we use a capital and lowercase Roman letter (e.g., $F$ and $f$) or Greek letters along with dot above (e.g., $\varphi$ and $\varphid$) to denote respectively absolutely continuous CDFs of arbitrary dimensions and the corresponding densities. When dealing with multivariate distributions, the marginal or conditional distribution over a subset of variables will be indicated by the argument names (i.e. $F(x_{1}|x_{2},x_{3})=\mathbb{P}\left[X_{1}\leq x_{1}|X_{2}=x_{2},X_{3}=x_{3}\right]$).

For a positive integer $p \in \N \setminus 0$, 
let $[p] = \{1, \dots, p\}$.
% If $S$ is a set, then $|S|$ and $S^{\times p}$ denote respectively its cardinality and the product set $S \times \cdots \times S$ with $|S^{\times p}| = |S|^p$.
Denote the space of absolutely continuous univariate and $d$-dimensional CDFs respectively by $\Fcal_1$ and $\Fcal_d$. 
% \begin{align*}
%      \Fcal_1 &= \{F \colon \R \to [0,1],\, \lim_{x \to -\infty} F(x) = 0,\, \lim_{x \to \infty} F(x) = 1,\, \partial F(x)/\partial x \ge 0 \},\\
%     \Fcal_d &= \{F \colon \R^d \to [0,1],\, \lim_{x_j \to -\infty} F(x_1, \dots, x_j, \dots, x_d) = 0\,\, \forall j \in [d],\, \lim_{x \to \infty} F(x, \dots, x) = 1, \\
%     &\phantom{\Fcal_d = \{F \colon \R^d \to [0,1]}\partial^{|k|} F(x_{1}, \dots, x_{d}) /\partial x_{i_{1}} \cdots \partial x_{i_{|k|}} \ge 0\,\, \forall k \subseteq [d]\}.
% \end{align*}
For any $F \in \Fcal_1$, the density $f:\R \to \R_{+}$ is $f(x) = \partial F(x)/\partial x$.
Similarly, for any $F \in \Fcal_d$, the density $f(\bm x):\R^d \to \R_{+}$ is $f(\bm x) = \partial^d F(\bm x)/\partial x_1 \cdots \partial x_d$,
and $F_j(x) = \lim_{z \to \infty} F(z, \dots, x, \dots, z) \in \Fcal_1$ for $j \in [d]$ is the $j$th marginal distribution.
% For an order $d$ tensor $A \in \R^{m_1 \times \cdots m_d}$, we use $\|A\|_1$ to denote the ``entrywise'' 1-norm, that is
% \begin{align*}
%     \|A\|_1 =\sum\limits_{i_1=1}^{m_1} \cdots \sum\limits_{i_d=1}^{m_d} |A_{i_1, \dots, i_d}|.
% \end{align*}

\subsection{The bivariate case}
For the task of modeling joint distributions of two variables supported on $\mathbb{R}^{2}$,
consider a family of univariate CDFs
$\{\varphi_{i,j}\,\}_{i\in[m],\,j\in[2]}$ with $\varphi_{i,j} \in \Fcal_1$, i.e., the functions 
$\varphi_{i,j}:\mathbb{R} \rightarrow [0,1]$ satisfy
\begin{align}
\varphi_{i,j}(-\infty) = 0 \,, \qquad     
\varphi_{i,j}(+\infty) = 1 \,, \qquad     
\dot{\varphi}_{i,j}(x_{j})  \geq 0 \,.
\end{align}
These functions will be our basic building block, 
and we model them using a simple neural architecture proposed in~\cite{balle2018variational}, which we review in~\Cref{app:univariate_marginal_param}. 
If $A$ is an $m \times m$ matrix of nonnegative elements satisfying $\sum_{i,j=1}^m A_{i,j} =1$,
we can combine it with the univariate CDFs to obtain
\begin{align} 
\label{eq:bivariate_cdf}
    F(x_{1},x_{2})=\sum\limits_{i,j=1}^{m} A_{i,j}\varphi_{i,1}(x_{1})\varphi_{j,2}(x_{2}).
\end{align}
The coefficients $A_{i,j}$ encode the dependencies between the two variables, and the normalization ensures that $F$ is a valid CDF, that is $F \in \Fcal_2$.
Even though in each summand the interaction is modeled by a single scalar parameter, such a model can be used to approximate well complex interactions between $x_1$ and $x_2$ if $m$ is sufficiently large, as we show in \Cref{sec:theory}. 
The advantage of this construction is that $\{\varphid_{i,j}\}_{i\in[m],\,j\in[2]}$, the family of densities corresponding to the univariate CDFs, leads immediately to 
\begin{align*}
f(x_{1},x_{2})=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2}). 
% f(x_{1},x_{2})=\partial^{2}F(x_{1},x_{2})/\partial x_{1}\partial x_{2}=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2}). 
\end{align*}
It is similarly straightforward to obtain marginal and conditional quantities, e.g.:
\begin{align*}
F(x_{1})&=\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1}), 
\qquad &f(x_{1})&=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1}),  \\
    F(x_{1}|x_{2})&=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})}, 
\qquad &f(x_{1}|x_{2})&=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})}.
    % F(x_{1})&=\lim_{x_2 \to \infty }F(x_{1},x_2)=\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1}), \\
    % F(x_{1}|x_{2})&=\frac{\partial F(x_{1},x_{2})/\partial x_{2}}{\partial F(x_{2}) /\partial x_{2}}=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})},
\end{align*}
Deriving these simple expressions 
relies on the fact that \eqref{eq:bivariate_cdf} combines the univariate CDFs linearly. Nonetheless, it is clear that, with $m \to \infty$ and for judiciously chosen univariate CDFs, such a model is a universal approximator of both CDFs and sufficiently smooth densities.

% And since evaluating the density requires taking derivatives with respect to all inputs, fully general nonlinear models can lead to a space and time complexity that is exponential in the number of variables.
% There is thus a tension between the ability to expressively model dependencies and obtain closed-form expressions for the density as well as all marginal and conditional quantities.


\subsection{The multivariate case}\label{sec:multivariate}

% \begin{figure}
%     \centering
%     \includegraphics[height=2in]{figs/tensors.jpg}
%     \caption{\textbf{Tensor decompositions}. a) Notation for tensors of various order (vectors, matrices, delta tensors). Each edge represents an index, and connecting two edges represents contraction (summation over an index). b) A general unstructured tensor of order d. c) The set of univariate CDFs. d)  
%     The CP decomposition and the hierarchical Tucker (HT) decomposition.}
%     \label{fig:tensor_decomps}
% \end{figure}

% Extending the above construction to the multivariate case, we are thus confronted with the problem of combining products of univariate CDFs linearly, in a manner that is both computationally efficient and expressive. %A sum over all possible products for example will require $n^d$ parameters and is thus impractical even for moderate $d$. 
% The linearity constraint reduces this to a tensor decomposition problem (with additional non-negativity and normalization constraints). There is an extensive literature on such efficient tensor decompositions (see \cite{Cichocki2017-gp} for a review). A graphical representation of the tensor decompositions used in this work is presented in \Cref{app:tensor_decomps}. %For example, a fundamental problem in many-body quantum mechanics is the efficient representation of the state of a many-body system, which is in fact a multivariate distribution, in terms of states of single particles defined in terms of univariate distributions. (add more examples?). 

% The analogy with tensor decompositions becomes clear when we consider discrete rather than continuous variables.
% Say we wish to model the joint distribution of $d$ discrete variables, each taking one of $S$ possible values.
% The distribution is then a function $\varphi_{S}:[S] \times \cdots \times [S] \rightarrow\mathbb{R}$, which can also be viewed as an order $d$ tensor.
% %We can represent tensors of any order graphically using standard notation in \cref{fig:tensor_decomps}a.
% A general tensor $\varphi_{S}$ %(as in the left of \cref{fig:tensor_decomps}b) 
% will require order of $S^d$ numbers to represent, and is thus impractical even for moderate $d$.
% The continuous analog of such a tensor is a multivariate function $F:\mathbb{R}^{d}\rightarrow\mathbb{R}$, with the value of $x_j$ corresponding to the discrete index $s_j$.
% We will thus use the same notation for the continuous case. 

To generalize the bivariate case, consider a collection of univariate CDFs $\{\varphi_{i,j}\}_{i\in[m],\,j\in[d]}$ with $\varphi_{i,j} \in \Fcal_1$ for each $i$ and $j$, and define the tensor-valued function $\Phi \colon \R^d \to [0,1]^m \times \cdots \times [0,1]^m$ by $\Phi(\bm x)_{i_1, \dots, i_d} = \prod_{j=1}^{d}\varphi_{i_{j},j}(x_{j})$ for $\bm x \in \R^d$.
Furthermore, denote the class of normalized order $d$ tensors with $m$ dimensions in each mode and nonnegative elements by
\begin{align}
    \Acal_{d,m} = \{A \in \R^{m \times \cdots \times m}\colon A_{i_1, \dots, i_d} \ge 0,\, \sum\limits_{i_1, \dots, i_d = 1}^m A_{i_1, \dots, i_d} = 1 \}.
    \label{eq:define_acal}
\end{align}
\begin{definition}[Marginalizable Distribution Model Approximator]
For $\Phi \colon \R^d \to [0,1]^m \times \cdots \times [0,1]^m$ as above and $A \in \Acal_{d,m}$,
the marginalizable distribution model approximator (MDMA) is
\begin{align} \label{eq:F_general_A}
    F_{A,\Phi}(\bm x)= \langle A, \Phi(\bm x) \rangle  = \sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\prod\limits_{j=1}^{d}\varphi_{i_{j},j}(x_{j}).
\end{align}
\end{definition}
If is clear that the conditions on $\Phi$ and $A$ imply that $F_{A,\Phi} \in \Fcal_d$.  
As in the bivariate case, densities or marginalization over $x_j$ are obtained by replacing each $\varphi_{i,j}$ respectively by $\varphid_{i,j}$ or $1$. 
As for conditioning, considering any disjoint subsets $R=\left\{ k_{1},\dots,k_{r}\right\}$ and $S=\left\{ j_{1},\dots,j_{s}\right\}$ of $[d]$ such that $R \cap S = \emptyset $, we have  
\begin{align*}
F_{A, \Phi}(x_{k_{1}},\dots,x_{k_{r}}|x_{j_{1}},\dots,x_{j_{s}}) & = \frac{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{k\in R}{\prod}\varphi_{i_{k},k}(x_{k})\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}.
%  f(x_{k_{1}},\dots,x_{k_{r}}|x_{j_{1}},\dots,x_{j_{s}}) &= \frac{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{k\in R}{\prod}\varphid_{i_{k}k}(x_{k})\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}.
\end{align*}
% and similarly the conditional density is obtained by replacing $\varphi_{i_{k},k}(x_{k})$ by $\varphid_{i_{k},k}(x_{k})$.

For a completely general tensor $A$, the expression \eqref{eq:F_general_A} is computationally impractical since such a model has $O(m^d)$ parameters, hence some structure must be imposed on $A$.
For instance, using $A_{i_1, \dots, i_d}=a_{i_1} \delta_{i_1, \dots, i_d}$ leads to $F_{A,\Phi}(\bm x)=\sum_{i=1}^m a_{i}\prod_{j=1}^{d}\varphi_{i,j}(x_{j})$, with $a_i \ge 0$ and $\sum_{i=1}^m a_{i} = 1$.
Instead this top-down approach, $A$ can be tractably constructed bottom-up, as we explain next. 
% A natural choice is the so-called order $m$ CP decomposition, given by
% \begin{align}\label{eq:CP}
%     F_{\mathrm{CP}}(x_{1},\dots,x_{d})=\sum\limits_{i=1}^m a_{i}\prod\limits_{j=1}^{d}\varphi_{i,j}(x_{j}),
% \end{align}
% where $a$ is an $m \times 1$ vector with nonnegative elements such that $\sum_{i=1}^m a_i=1$.
% This is clearly a valid CDF and can be made more expressive by increasing $m$. 
% A more powerful parametrization of $A$ is a variant of the hierarchical Tucker (HT) decomposition first introduced in \cite{Hackbusch2009-yr}%, which we illustrate in \Cref{fig:tensor_decomps}e.
% Such tensors were used in the construction of deep linear convolutional networks for image classification in \cite{cohen2016expressive}.
% Specifically, we take the coefficients in \cite{Hackbusch2009-yr} to be diagonal with respect to their lower indices and fix the pool size as 2, yet for brevity refer to such a decomposition henceforth as the HT decomposition.
% Fixing a pool size 2 and 

Assuming for simplicity that $d$ is an integer power of 2, let $\varphi^{1} \colon \R^d \to \R^{m \times d}$ be the matrix-valued function defined by $\varphi^{1}_{i,j}(\bm x) = \varphi_{i,j}(x_j)$.
For $l \in \{2, \dots, \log_2 d\}$, define the matrix-value functions $\varphi^{l}\colon \R^d \to \R^{m \times d/2^{l-1}}$ recursively by 
\begin{align}\label{eq:HT_recurs}
\varphi_{i,j}^{l}(\bm{x})=\sum\limits _{k=1}^{m}\lambda_{i,k,j}^{l-1}\varphi_{k,2j-1}^{l-1}(\bm{x})\varphi_{k,2j}^{l-1}(\bm{x}),
\end{align}
where $\lambda^{l}$ is an $m \times m \times d/2^{l}$ tensor.
The CDF can then be written as
\begin{align} \label{eq:HT}
 F_{A, \Phi}(\bm x) &= \sum\limits_{k=1}^m a_{k} \varphi_{k,1}^{\log_{2}d}(\bm x)\varphi_{k,2}^{\log_{2}d}(\bm x),
\end{align}
with $a \in \mathbb{R}^m$. %an $m \times 1$ vector as in \eqref{eq:CP}.
If all parameters are nonnegative, $\sum_{k=1}^m \lambda_{i,k,j}^{l}=1$ for all $l$, and $\sum_{k=1}^m a_k=1$, it is easy to verify that the underlying $A$ satisfies $A \in \Acal_{d,m}$ defined in (\ref{eq:define_acal}). 
As a concrete example, for $d=4$, we have 
\begin{align*}
% F_{\mathrm{HT}}(\bm x)  
%   &= \sum\limits_{k_1,k_2,k_2'=1}^m a_{k_1} \lambda_{k_2,k_1,1}^{1}\lambda_{k_2',k_1,2}^{1}\varphi_{k_2,1}^{1}(\bm x)\varphi_{k_2,2}^{1}(\bm x)\varphi_{k_2',3}^{1}(\bm x)\varphi_{k_2',4}^{1}(\bm x) 
F_{A, \Phi}(\bm{x})=\sum\limits _{k_{2},k_{1},k_{1}'=1}^{m}a_{k_{2}}\lambda_{k_{2},k_{1},1}^{1}\lambda_{k_{2},k_{1}',2}^{1}\varphi_{k_{1},1}^{1}(\bm{x})\varphi_{k_{1},2}^{1}(\bm{x})\varphi_{k_{1}',3}^{1}(\bm{x})\varphi_{k_{1}',4}^{1}(\bm{x})
\end{align*}
from which we can read off that $A_{i_{1},i_{2},i_{3},i_{4}}=\sum_{k=1}^{m}a_{k}\lambda_{k,i_{1},1}^{1}\lambda_{k,i_{3},2}^{1}\delta_{i_{1},i_{2}}\delta_{i_{3},i_{4}}$. Note that the number of parameters required to represent $A$ is only $\mathrm{poly}(m,d)$.
The construction can be generalized straightforwardly to cases where $d$ is not divisible by 2, and/or the pool size is any positive integer.
It is in fact a variant of the hierarchical Tucker decomposition \cite{Hackbusch2009-yr}, which has been used in the construction of tensor networks for image classification in \cite{cohen2016expressive}.  
A graphical representation of this tensor is provided in \Cref{fig:tensor_decomps} in the supplementary materials.  
We present additional details regarding the choice of architecture and initialization in \Cref{app:design_details}. 

\subsection{A non-marginalizable variant} \label{sec:nmdma}

We can construct a more expressive variant of MDMA at the price of losing the ability to marginalize and condition on arbitrary subsets of variables. We find that the resulting model leads to state-of-the-art performance on a density estimation benchmark.
We define $\mathbf{v}=\mathbf{x}+\mathbf{T}\sigma(\mathbf{x})$ where $\mathbf{T}$ is an upper-triangular matrix with non-negative entries and $0$ on the main diagonal. Note that $\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}}\right|=1$.
Given some density $f(v_{1},\dots,v_{d})=\prod\limits_{j=1}^{d}\varphid_{j}(v_{j})$, we have 
\begin{align}
f(x_{1},\dots,x_{d})=\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}}\right|f(v_{1},\dots,v_{d})=f(v_{1}(\mathbf{x}),\dots,v_{d}(\mathbf{x})).
\end{align}
We refer to this model nMDMA, since it is \textit{non}-marginalizable.  
% {\color{red}
% It follows that 
% \eqan
% F(x_{1},\dots,x_{d})&=&\int_{-\infty}^{\mathbf{x}}\prod\limits_{j=1}^{d}dx_{j}'f(x'_{1},\dots,x'_{d})\\
% &=&\int_{-\infty}^{\mathbf{x}}\prod\limits_{j=1}^{d}dx'_{j}\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}'}\right|f(v_{1}(\mathbf{x}'),\dots,v_{d}(\mathbf{x}'))\\
% &=&\int_{-\infty}^{\mathbf{v}(\mathbf{x})}\prod\limits_{j=1}^{d}dv'_{j}f(v'_{1},\dots,v'_{d})\\
% &=&\prod\limits_{j=1}^{d}\varphi_{j}(v_{j}(\mathbf{x})).
% \enan
% Marginalizing over a subset of the $x_j$ is done by setting these variables to $\infty$ in the expression $\underset{j=1}{\overset{d}{\Pi}}\varphi_{j}(v_{j}(\mathbf{x}))$. The marginal density can be obtained by taking derivatives of the marginal CDF. For a block-triangular matrix with block size $S$ this will generate no more than $Sd$ terms. Conditional PDFs and CDFs can be obtained from the marginals and the joints as before. 

% We can also include permutations to group the variables in different ways. 
% % In order to combine this approach with the HT decomposition of the tensor $A$, we simply set the permutation matrix $P$ to be an identity. This ensures that each summand in the expression $\left\langle A,\Phi(\mathbf{y})\right\rangle $ is a valid CDF.  
% }
% \subsection{A simple example}
% Consider the transformation 
% \eqan 
% v_1 &=& x_1
% \\
% v_2 &=& \alpha \sigma(x_1) + x_2
% \enan 
% We model the CDF of $(v_1,v_2)$ as
% \eqan 
% F(v_1,v_2) = \phi_{1}(v_1) \phi_2(v_2)
% \label{eq:CD\varphi_v}
% \enan
% and the pdfs is
% \eqan 
% p(x_1,x_2) &=& p(v_1,v_2) 
% \\
% &=&  \phi_{1}'(v_1) \phi_2'(v_2)
% \\
% &=& \phi_{1}'(x_1) \phi_2'(\alpha \sigma(x_1) + x_2)
% \label{eq:density_v}
% \enan 
% where we used that the 
% Jacobian is unity. 

% To obtain the marginal $p(x_2)$, we start 
% with the CFD
% \eqan 
% F(x_2, x_1=\infty) = \phi_2(\alpha +x_2),
% \enan 
% where we used (\ref{eq:CD\varphi_v}), 
% and take the derivative w.r.t. $x_2$,
% \eqan 
% p(x_2) = \phi_2'(\alpha +x_2)\,.
% \enan 
% To verify that this expression is consistent with (\ref{eq:density_v}), note that 
% \eqan 
% \int_{-\infty}^{+\infty}dx'_1 p(x'_1,x_2) &=& \int_{-\infty}^{+\infty}dx'_1\phi_{1}'(x'_1) \phi_2'(\alpha \sigma(x'_1) + x_2)
% \\
% &=& \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{+\infty}dx'_1
% \int_{-\infty}^{+x_2}dx'_2
% \phi_{1}'(x'_1) 
% \phi_2'(\alpha \sigma(x'_1) + x_2')
% \\
% &=&
% \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{+\infty}dv'_1
% \int_{-\infty}^{\alpha +x_2  }dv'_2
% \phi_{1}'(v'_1) 
% \phi_2'(v_2')
% \\
% &=&
% \int_{-\infty}^{+\infty}dv'_1
% \phi_{1}'(v'_1) 
% \, \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \\
% &=& \phi_2'(\alpha + x_2)
% \enan 

% \subsubsection*{Three variables}
% \eqan 
% p(x_1,x_2,x_3) &=& p(v_1,v_2,v_3) 
% \\
% &=&  \phi_{1}'(v_1) \phi_2'(v_2) \phi_3'(v_3)
% \\
% &=& \phi_{1}'(x_1) \phi_2'(\alpha \sigma(x_1) + x_2)
% \phi_3'(\alpha_{31} \sigma(x_1) + \alpha_{32} \sigma(x_2) + x_3)
% \label{eq:density_v3}
% \enan 
% where we used that the 
% Jacobian is unity. 

% % To obtain the marginal $p(x_2,x_3)$, we start 
% % with the CFD
% % \eqan 
% % F(x_2, x_1=\infty) = \phi_2(\alpha +x_2),
% % \enan 
% % where we used (\ref{eq:CD\varphi_v}), 
% % and take the derivative w.r.t. $x_2$,
% % \eqan 
% % p(x_2) = \phi_2'(\alpha +x_2)\,.
% % \enan 
% % To verify that this expression is consistent with (\ref{eq:density_v}), note that 
% {\tiny 
% \eqan 
% \int_{-\infty}^{+\infty}dx'_1 p(x'_1,x_2,x_3) &=&
% \int_{-\infty}^{+\infty}dx'_1
% \phi_{1}'(x_1') \phi_2'(\alpha \sigma(x_1') + x_2)
% \phi_3'(\alpha_{31} \sigma(x_1') + \alpha_{32} \sigma(x_2) + x_3)
% \nn 
% \\
% &=& \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{+\infty}dx'_1
% \int_{-\infty}^{+x_2}dx'_2
% \int_{-\infty}^{+x_3}dx'_3
% \phi_{1}'(x_1') \phi_2'(\alpha \sigma(x_1') + x_2')
% \phi_3'(\alpha_{31} \sigma(x_1') + \alpha_{32} \sigma(x_2') + x_3')
% \nn 
% \\
% &=&
% \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{+\infty}dv'_1
% \int_{-\infty}^{\alpha +x_2  }dv'_2
% \int_{-\infty}^{\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3 }dv'_3
% \phi_{1}'(v'_1) 
% \phi_2'(v_2')
% \phi_3'(v_3')
% \\
% &=&
% \int_{-\infty}^{+\infty}dv'_1
% \phi_{1}'(v'_1) 
% \, 
% \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \int_{-\infty}^{\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3 }dv'_3 \phi_3'(v_3')
% \\
% &=& 
% \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \phi_3'(\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3)
% \\
% &=& 
% \frac{\partial}{\partial x_2} 
% \left[ 
% \phi_2(\alpha + x_2)
% \phi_3'(\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3)
% \right]
% \enan 
% }


\subsection{Efficient sampling}
{\color{red}TODO: update notation}

{\color{red}can drop this paragraph}
Given a model of a multivariate CDF \cref{eq:F_general_A} we can readily compute the conditional univariate CDFs and invert them numerically, which allows for sampling in the same manner as other autoregressive models.
To be precise, sampling a vector $(u_{1},\dots,u_{d})$ of independent components from the uniform distribution, we obtain a sample from $F$ by computing 
\begin{equation}
x_{1} =F_{A,\Phi}^{-1}(u_{1}),\quad x_{i} = F_{A,\Phi}^{-1}(u_{i}|x_{1},\dots,x_{i-1}),
\end{equation}
(where unlike other autoregressive model, the order of taking the conditionals need not be fixed).
The main drawback of this method is that due to the sequential nature of the sampling the computational cost is linear in $d$ and cannot be parallelized.
In addition, evaluation of the inverse conditional CDFs requires evaluating multiple forward passes of the model. 

However, the structure of $F_{A,\Phi}$ defined in \cref{eq:F_general_A} can be leveraged to sample much more efficiently.
Define by $R_{A}$ a vector-valued categorical random variable taking values in $\left[m\right]^{\times d}$, with distribution 
\begin{equation}
    \mathbb{P}\left[R_{A}=(i_{1},\dots,i_{d})\right]=A_{i_{1},\dots,i_{d}}.
\end{equation}
The fact that $A$ is nonnegative and satisfies $\|A\|_1=1$ ensure the validity of this definition.
Consider a vector $(\tilde{X}_{1},\dots,\tilde{X}_{d},R_{A})$ where $R_A$ is distributed as above, and 
\begin{equation}
    \mathbb{P}\left[\tilde{X}_{1}\leq x_{1},\dots,\tilde{X}_{d}\leq x_{d}|R_{A}=\mathbf{r}\right]=\prod\limits_{i=1}^{d}\varphi_{r_{i},i}(x_{i}),
\end{equation}
for a collection $\{\varphi_{i,j}\}$ of univariate CDFs. Denoting the distribution of this vector by $\tilde{F}_{A,\Phi}$, marginalizing over $R_A$ gives 
\begin{equation}
	\tilde{F}_{A,\Phi}(x_{1},\dots,x_{d})=\underset{\mathbf{r}\in[m]^{d}}{\sum}\mathbb{P}\left[R_{A}=\mathbf{r}\right]\prod\limits_{j=1}^{d}\varphi_{r_{j},j}(x_{j})
	%=\underset{i_{1},\dots,i_{d}=1}{\overset{m}{\sum}}A_{i_{1},\dots,i_{d}}\prod\limits_{i=1}^{d}\varphi_{i_{j},j}(x_{j})
	=F_{A,\Phi}(x_{1},\dots,x_{d}).
\end{equation}
Instead of sampling directly from the distribution $F_{A,\Phi}$, we can thus sample from $\tilde{F}_{A,\Phi}(x_{1},\dots,x_{d})$ and discard the sample of $R_A$. To do this, we first sample from the categorical variable $R_A$. Denoting this sample by $\mathbf{r}$, we can sample from $\tilde{X}_{i}$ by inverting the univariate CDF $\varphi_{r_{i},i}$. This can be done \textit{in parallel} for all $i$. 

The approach outlined above is impractical since $R_{A}$ can take $m^d$ possible values, yet if $A$ can be expressed by an efficient tensor representation this exponential dependence can be avoided. Consider the HT decomposition \cref{eq:HT}. It can be written as 
\begin{equation}
\left\langle A,\Phi\right\rangle =\underset{\ell,j_{\ell}}{\prod}\underset{k_{\ell,j_{\ell}}=1}{\overset{m_{\ell}}{\sum}}a_{k_{\ell-1,\left\lceil j_{\ell}/2\right\rceil },j_{\ell}}^{\ell,k_{\ell,j_{\ell}}}\Phi_{k_{1,1},\dots,k_{1,\left\lceil d/2\right\rceil }}.
\end{equation}
%which is a normalized sum of $O(md)$ CDFs. We can sample from this mixture in $O(\log d)$ time and requiring the storage of only $O(d)$ integers. 

Define a collection of independent categorical variables $\{R^\ell_{i,j}\}$ taking values in $[m_\ell]$, such that 
\begin{equation}
	\forall\ell,i,j:\quad\mathbb{P}\left[R_{i,j}^{\ell}=k\right]=a_{i,j}^{\ell,k},
\end{equation}
where $\left\{ a_{i,j}^{\ell,k}\right\}$ are the parameters of the HT decomposition (our normalization of the HT coefficients ensures that this is a valid distribution).

If we define a random vector $(\tilde{X}_{1},\dots,\tilde{X}_{d})$ as before such that
\begin{equation}
\mathbb{P}\left[\tilde{X}_{1}\leq x_{1},\dots,\tilde{X}_{d}\leq x_{d}|R^{1}=\mathbf{k}_{1}\cap R^{2}=\mathbf{k}_{2}\cap\dots\cap R^{\ell_{d}}=k_{\ell_{d}}\right]=\prod\limits _{i=1}^{d}\varphi_{k_{1,i/2},i}(x_{i}),
\end{equation}
 we again find that the distribution of $(\tilde{X}_{1},\dots,\tilde{X}_{d})$ obtained by marginalizing over $\{R^\ell_{i,j}\}$ is equal to $F_{\mathrm{HT}}$, hence we can sample from $(\tilde{X}_{1},\dots,\tilde{X}_{d},\{R_{i,j}^{\ell}\})$ instead.

Sampling $\{R_{i,j}^{\ell}\}$ is best done sequentially starting from the final layer. We first sample from $R^{\ell_d}$ obtaining a sample $k_{\ell_d}$. We next sample from $R_{k_{\ell_{d}},1}^{\ell_{d}-1},R_{k_{\ell_{d}},2}^{\ell_{d}-1}$ obtaining samples $k_{\ell_{d}-1,1},k_{\ell_{d}-1,2}$ and proceed similarly until the reaching the first layer. There are $\left\lceil \log_2 d\right\rceil $ layers in the decomposition, and aside from storing the decomposition itself this sampling procedure requires storing only $O(d)$ integers. Since 
\begin{equation}
	\mathbb{P}\left[R^{\ell_{d}}=k_{\ell_{d}}\cap R_{k_{\ell_{d}},1}^{\ell_{d}-1}=k_{\ell_{d}-1,1}\cap R_{k_{\ell_{d}},2}^{\ell_{d}-1}=k_{\ell_{d}-1,2},\dots,R_{k_{2,d/2},d/2}^{1}=k_{1,d/2}\right]=\underset{\ell,j_{\ell}}{\prod}a_{k_{\ell-1,\left\lceil j_{\ell}/2\right\rceil },j_{\ell}}^{\ell,k_{\ell,j_{\ell}}},
\end{equation}
sampling from the categorical variables in this fashion is equivalent to sampling a mixture component. We then sample $\tilde{X}_{i}$ by inverting the univariate CDF $\varphi_{k_{1,\left\lceil i/2\right\rceil },i}(x_{i})$, parallelizing over $i$. Note that the time complexity of this sampling depends only logarithmically on $d$, and this logarithmic dependence is only in the sampling from the categorical variables which is inexpensive to begin with. We thus avoid the linear dependence on $d$ that is common in sampling from autoregressive models. 


==> Marginalizable Density Models (4)/arxiv/mdma2.tex <==
%!TEX root = ../MDN_neurips.tex

\section{Marginalizable Density Models}
\label{sec:marginalizable_models}

\subsection{Notations}
In the following, we use a capital and lowercase Roman letter (e.g., $F$ and $f$) or Greek letters along with dot above (e.g., $\varphi$ and $\varphid$) to denote respectively absolutely continuous CDFs of arbitrary dimensions and the corresponding densities. When dealing with multivariate distributions, the marginal or conditional distribution over a subset of variables will be indicated by the argument names (i.e., $F(x_{1}|x_{2},x_{3})=\mathbb{P}\left[X_{1}\leq x_{1}|X_{2}=x_{2},X_{3}=x_{3}\right]$).

For a positive integer $p \in \N \setminus 0$, 
let $[p] = \{1, \dots, p\}$.
% If $S$ is a set, then $|S|$ and $S^{\times p}$ denote respectively its cardinality and the product set $S \times \cdots \times S$ with $|S^{\times p}| = |S|^p$.
Denote the space of absolutely continuous univariate and $d$-dimensional CDFs respectively by $\Fcal_1$ and $\Fcal_d$. 
% \begin{align*}
%      \Fcal_1 &= \{F \colon \R \to [0,1],\, \lim_{x \to -\infty} F(x) = 0,\, \lim_{x \to \infty} F(x) = 1,\, \partial F(x)/\partial x \ge 0 \},\\
%     \Fcal_d &= \{F \colon \R^d \to [0,1],\, \lim_{x_j \to -\infty} F(x_1, \dots, x_j, \dots, x_d) = 0\,\, \forall j \in [d],\, \lim_{x \to \infty} F(x, \dots, x) = 1, \\
%     &\phantom{\Fcal_d = \{F \colon \R^d \to [0,1]}\partial^{|k|} F(x_{1}, \dots, x_{d}) /\partial x_{i_{1}} \cdots \partial x_{i_{|k|}} \ge 0\,\, \forall k \subseteq [d]\}.
% \end{align*}
For any $F \in \Fcal_1$, the density $f:\R \to \R_{+}$ is $f(x) = \partial F(x)/\partial x$.
Similarly, for any $F \in \Fcal_d$, the density $f(\bm x):\R^d \to \R_{+}$ is $f(\bm x) = \partial^d F(\bm x)/\partial x_1 \cdots \partial x_d$,
and $F_j(x) = \lim_{z \to \infty} F(z, \dots, x, \dots, z) \in \Fcal_1$ for $j \in [d]$ is the $j$th marginal distribution.
% For an order $d$ tensor $A \in \R^{m_1 \times \cdots m_d}$, we use $\|A\|_1$ to denote the ``entrywise'' 1-norm, that is
% \begin{align*}
%     \|A\|_1 =\sum\limits_{i_1=1}^{m_1} \cdots \sum\limits_{i_d=1}^{m_d} |A_{i_1, \dots, i_d}|.
% \end{align*}

\subsection{The bivariate case}
For the task of modeling joint distributions of two variables supported on $\mathbb{R}^{2}$,
consider a family of univariate CDFs
$\{\varphi_{i,j}\,\}_{i\in[m],\,j\in[2]}$ with $\varphi_{i,j} \in \Fcal_1$, i.e., the functions 
$\varphi_{i,j}:\mathbb{R} \rightarrow [0,1]$ satisfy
\begin{align*}
\lim_{x\to -\infty}\varphi_{i,j}(x) = 0 \,, \qquad     
\lim_{x\to \infty}\varphi_{i,j}(x) = 1 \,, \qquad     
\varphid_{i,j}(x) = \partial \varphi(x) / \partial x  \geq 0 \,.
\end{align*}
These functions are our basic building block, 
and we model them using a simple neural architecture proposed in~\cite{balle2018variational} and described in~\Cref{sec:theory}. 
If $A$ is an $m \times m$ matrix of nonnegative elements satisfying $\sum_{i,j=1}^m A_{i,j} =1$,
we can combine it with the univariate CDFs to obtain
\begin{align} 
\label{eq:bivariate_cdf}
    F(x_{1},x_{2})=\sum\limits_{i,j=1}^{m} A_{i,j}\varphi_{i,1}(x_{1})\varphi_{j,2}(x_{2}).
\end{align}
The coefficients $A_{i,j}$ encode the dependencies between the two variables, and the normalization ensures that $F$ is a valid CDF, that is $F \in \Fcal_2$.
Even though in each summand the interaction is modeled by a single scalar parameter, such a model can be used to approximate well complex interactions between $x_1$ and $x_2$ if $m$ is sufficiently large, as we show in \Cref{sec:theory}. 
The advantage of this construction is that $\{\varphid_{i,j}\}_{i\in[m],\,j\in[2]}$, the family of densities corresponding to the univariate CDFs, leads immediately to 
\begin{align*}
f(x_{1},x_{2})=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2}). 
% f(x_{1},x_{2})=\partial^{2}F(x_{1},x_{2})/\partial x_{1}\partial x_{2}=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2}). 
\end{align*}
It is similarly straightforward to obtain marginal and conditional quantities, e.g.:
\begin{align*}
F(x_{1})&=\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1}), \qquad
%  &f(x_{1})&=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1}),  \\
    F(x_{1}|x_{2})=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})}, 
% \qquad &f(x_{1}|x_{2})&=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})}.
    % F(x_{1})&=\lim_{x_2 \to \infty }F(x_{1},x_2)=\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1}), \\
    % F(x_{1}|x_{2})&=\frac{\partial F(x_{1},x_{2})/\partial x_{2}}{\partial F(x_{2}) /\partial x_{2}}=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})},
\end{align*}
and the corresponding densities result from replacing $\varphi_{i,1}$ by $\varphid_{i,1}$.
Deriving these simple expressions 
relies on the fact that \eqref{eq:bivariate_cdf} combines the univariate CDFs linearly. Nonetheless, it is clear that, with $m \to \infty$ and for judiciously chosen univariate CDFs, such a model is a universal approximator of both CDFs and sufficiently smooth densities.

% And since evaluating the density requires taking derivatives with respect to all inputs, fully general nonlinear models can lead to a space and time complexity that is exponential in the number of variables.
% There is thus a tension between the ability to expressively model dependencies and obtain closed-form expressions for the density as well as all marginal and conditional quantities.


\subsection{The multivariate case}\label{sec:multivariate}

% \begin{figure}
%     \centering
%     \includegraphics[height=2in]{figs/tensors.jpg}
%     \caption{\textbf{Tensor decompositions}. a) Notation for tensors of various order (vectors, matrices, delta tensors). Each edge represents an index, and connecting two edges represents contraction (summation over an index). b) A general unstructured tensor of order d. c) The set of univariate CDFs. d)  
%     The CP decomposition and the hierarchical Tucker (HT) decomposition.}
%     \label{fig:tensor_decomps}
% \end{figure}

% Extending the above construction to the multivariate case, we are thus confronted with the problem of combining products of univariate CDFs linearly, in a manner that is both computationally efficient and expressive. %A sum over all possible products for example will require $n^d$ parameters and is thus impractical even for moderate $d$. 
% The linearity constraint reduces this to a tensor decomposition problem (with additional non-negativity and normalization constraints). There is an extensive literature on such efficient tensor decompositions (see \cite{Cichocki2017-gp} for a review). A graphical representation of the tensor decompositions used in this work is presented in \Cref{app:tensor_decomps}. %For example, a fundamental problem in many-body quantum mechanics is the efficient representation of the state of a many-body system, which is in fact a multivariate distribution, in terms of states of single particles defined in terms of univariate distributions. (add more examples?). 

% The analogy with tensor decompositions becomes clear when we consider discrete rather than continuous variables.
% Say we wish to model the joint distribution of $d$ discrete variables, each taking one of $S$ possible values.
% The distribution is then a function $\varphi_{S}:[S] \times \cdots \times [S] \rightarrow\mathbb{R}$, which can also be viewed as an order $d$ tensor.
% %We can represent tensors of any order graphically using standard notation in \cref{fig:tensor_decomps}a.
% A general tensor $\varphi_{S}$ %(as in the left of \cref{fig:tensor_decomps}b) 
% will require order of $S^d$ numbers to represent, and is thus impractical even for moderate $d$.
% The continuous analog of such a tensor is a multivariate function $F:\mathbb{R}^{d}\rightarrow\mathbb{R}$, with the value of $x_j$ corresponding to the discrete index $s_j$.
% We will thus use the same notation for the continuous case. 

To generalize the bivariate case, consider a collection of univariate CDFs $\{\varphi_{i,j}\}_{i\in[m],\,j\in[d]}$ with $\varphi_{i,j} \in \Fcal_1$ for each $i$ and $j$, and define the tensor-valued function $\Phi \colon \R^d \times [m]^d \to [0,1]$ by $\Phi(\bm x)_{i_1, \dots, i_d} = \prod_{j=1}^{d}\varphi_{i_{j},j}(x_{j})$ for $\bm x \in \R^d$.
Furthermore, denote the class of normalized order $d$ tensors with $m$ dimensions in each mode and nonnegative elements by
\begin{align}
    \Acal_{d,m} = \{A \in \R^{m \times \cdots \times m}\colon A_{i_1, \dots, i_d} \ge 0,\, \sum\limits_{i_1, \dots, i_d = 1}^m A_{i_1, \dots, i_d} = 1 \}.
    \label{eq:define_acal}
\end{align}
\begin{definition}[Marginalizable Density Model Approximator]
For $\Phi \colon \R^d \times [m]^d \to [0,1]$ as above and $A \in \Acal_{d,m}$,
the marginalizable density model approximator (MDMA) is
\begin{align} \label{eq:F_general_A}
    F_{A,\Phi}(\bm x)= \langle A, \Phi(\bm x) \rangle  = \sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\prod\limits_{j=1}^{d}\varphi_{i_{j},j}(x_{j}).
\end{align}
\end{definition}
If is clear that the conditions on $\Phi$ and $A$ imply that $F_{A,\Phi} \in \Fcal_d$.  
As in the bivariate case, densities or marginalization over $x_j$ are obtained by replacing each $\varphi_{i,j}$ respectively by $\varphid_{i,j}$ or $1$. 
As for conditioning, considering any disjoint subsets $R=\left\{ k_{1},\dots,k_{r}\right\}$ and $S=\left\{ j_{1},\dots,j_{s}\right\}$ of $[d]$ such that $R \cap S = \emptyset $, we have  
\begin{align*}
F_{A, \Phi}(x_{k_{1}},\dots,x_{k_{r}}|x_{j_{1}},\dots,x_{j_{s}}) & = \frac{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{k\in R}{\prod}\varphi_{i_{k},k}(x_{k})\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}.
%  f(x_{k_{1}},\dots,x_{k_{r}}|x_{j_{1}},\dots,x_{j_{s}}) &= \frac{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{k\in R}{\prod}\varphid_{i_{k}k}(x_{k})\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}.
\end{align*}
% and similarly the conditional density is obtained by replacing $\varphi_{i_{k},k}(x_{k})$ by $\varphid_{i_{k},k}(x_{k})$.

For a completely general tensor $A$
with $m^d$ parameters, the expression \eqref{eq:F_general_A} is computationally impractical, hence some structure must be imposed on $A$.
For instance, one simple choice is $A_{i_1, \dots, i_d}=a_{i_1} \delta_{i_1, \dots, i_d}$, which leads to $F_{A,\Phi}(\bm x)=\sum_{i=1}^m a_{i}\prod_{j=1}^{d}\varphi_{i,j}(x_{j})$, with $a_i \ge 0$ and $\sum_{i=1}^m a_{i} = 1$.
Instead of this top-down approach, $A$ can be tractably constructed bottom-up, as we explain next. 
% A natural choice is the so-called order $m$ CP decomposition, given by
% \begin{align}\label{eq:CP}
%     F_{\mathrm{CP}}(x_{1},\dots,x_{d})=\sum\limits_{i=1}^m a_{i}\prod\limits_{j=1}^{d}\varphi_{i,j}(x_{j}),
% \end{align}
% where $a$ is an $m \times 1$ vector with nonnegative elements such that $\sum_{i=1}^m a_i=1$.
% This is clearly a valid CDF and can be made more expressive by increasing $m$. 
% A more powerful parametrization of $A$ is a variant of the hierarchical Tucker (HT) decomposition first introduced in \cite{Hackbusch2009-yr}%, which we illustrate in \Cref{fig:tensor_decomps}e.
% Such tensors were used in the construction of deep linear convolutional networks for image classification in \cite{cohen2016expressive}.
% Specifically, we take the coefficients in \cite{Hackbusch2009-yr} to be diagonal with respect to their lower indices and fix the pool size as 2, yet for brevity refer to such a decomposition henceforth as the HT decomposition.
% Fixing a pool size 2 and 

Assuming 
$d=2^p$ for integer~$p$, 
define $\varphi^{\ell}\colon \R^d \to \R^{m \times 2^{p-\ell+1}}$
for $\ell \in \{ 1, \dots, p \}$ recursively by
\begin{align}\label{eq:HT_recurs}
\varphi_{i,j}^{\ell}(\bm{x}) & = 
\begin{cases}
\varphi_{i,j}(x_j), \qquad &\ell = 1 \\
\sum\limits _{k=1}^{m}\lambda_{i,k,j}^{\ell-1}\varphi_{k,2j-1}^{\ell-1}(\bm{x})\varphi_{k,2j}^{\ell-1}(\bm{x}), \qquad &\ell  = 2, \dots, p
\end{cases}
\end{align} 
for $i \in [m]$, $j \in [2^{p-\ell +1}]$, and where $\lambda^{\ell}$ is a non-negative $m \times m \times 2^{p-\ell+1}$ tensor, normalized as $\sum_{k=1}^m \lambda_{i,k,j}^{\ell}=1$. 
The joint CDF can then be written as
\begin{align} 
\label{eq:HT}
 F_{A^{\mathrm{HT}}, \Phi}(\bm x) &= \sum\limits_{k=1}^m \lambda_{k}^{p} \varphi_{k,1}^{p}(\bm x)\varphi_{k,2}^{p}(\bm x),
\end{align}
with $\lambda^p \in \mathbb{R}_{+}^{m}$ satisfying $\sum_{k=1}^m \lambda_k^p=1$. 
It is easy to verify that the underlying $A^{\mathrm{HT}}$ satisfies $A^{\mathrm{HT}} \in \Acal_{d,m}$ defined in \eqref{eq:define_acal}. A graphical representation of this tensor is provided in \Cref{fig:tensor_decomps} in the supplementary materials.  

For example, for $d=4$, we first combine $(x_1,x_2)$ and $(x_3,x_4)$ into
\begin{align*}
    \varphi^2_{i,1}(\bm{x}) = \sum_{k=1}^m \lambda^1_{i,k,1} \varphi_{k,1}(x_1) \varphi_{k,2}(x_2) \,,
    \qquad 
    \varphi^2_{i,2}(\bm{x}) = \sum_{k=1}^m \lambda^1_{i,k,2} \varphi_{k,3}(x_3) \varphi_{k,4}(x_4) \,, 
\end{align*}
and then merge them as 
\begin{align}
F_{A^{\mathrm{HT}},\Phi} (\bm{x}) =    \sum_{k=1}^m \lambda_k^2 \varphi^2_{k,1}(\bm{x}) \varphi^2_{k,2}(\bm{x}),
\end{align}
from which we can read off that $A^{\mathrm{HT}}_{i_{1},i_{2},i_{3},i_{4}}=\sum_{k=1}^{m}\lambda_{k}^2\lambda_{k,i_{1},1}^{1}\lambda_{k,i_{3},2}^{1}\delta_{i_{1},i_{2}}\delta_{i_{3},i_{4}}$. 

Note that the number of parameters required to represent $A^{\mathrm{HT}}$ is only $\mathrm{poly}(m,d)$. The construction is easily 
generalized to dimensions $d$ not divisible by 2. 
Also, the number of $\varphi$ factors combined at 
each iteration in (\ref{eq:HT_recurs}) (called the \emph{pool size}),
 can be any positive integer.
 This construction is a variant of the hierarchical Tucker decomposition of tensors~\cite{Hackbusch2009-yr}, which has been used in the construction of tensor networks for image classification in \cite{cohen2016expressive}.  

Given a set of training points $\{\bm{x} \}_{i=1}^{N}$, we fit
MDMA models by maximizing the log of the density with respect to both the parameters in $\{ \varphi_{i,j}\}_{i\in[m],j\in[d]}$ and the components of $A$. We present additional details regarding the choice of architectures and initialization in \Cref{app:design_details}. 


\subsection{A non-marginalizable MDMA} \label{sec:nmdma}

We can construct a more expressive variant of MDMA at the price of losing the ability to marginalize and condition on arbitrary subsets of variables. We find that the resulting model leads to state-of-the-art performance on a density estimation benchmark.
We define $\mathbf{v}=\mathbf{x}+\mathbf{T}\sigma(\mathbf{x})$ where $\mathbf{T}$ is an upper-triangular matrix with non-negative entries and $0$ on the main diagonal. Note that $\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}}\right|=1$.
Given some density $f(v_{1},\dots,v_{d})=\prod\limits_{j=1}^{d}\varphid_{j}(v_{j})$, we have 
\begin{align}
f(x_{1},\dots,x_{d})=\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}}\right|f(v_{1},\dots,v_{d})=f(v_{1}(\mathbf{x}),\dots,v_{d}(\mathbf{x})).
\end{align}
We refer to this model nMDMA, since it no longer enables efficient marginalization and conditioning. 
% {\color{red}
% It follows that 
% \eqan
% F(x_{1},\dots,x_{d})&=&\int_{-\infty}^{\mathbf{x}}\prod\limits_{j=1}^{d}dx_{j}'f(x'_{1},\dots,x'_{d})\\
% &=&\int_{-\infty}^{\mathbf{x}}\prod\limits_{j=1}^{d}dx'_{j}\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}'}\right|f(v_{1}(\mathbf{x}'),\dots,v_{d}(\mathbf{x}'))\\
% &=&\int_{-\infty}^{\mathbf{v}(\mathbf{x})}\prod\limits_{j=1}^{d}dv'_{j}f(v'_{1},\dots,v'_{d})\\
% &=&\prod\limits_{j=1}^{d}\varphi_{j}(v_{j}(\mathbf{x})).
% \enan
% Marginalizing over a subset of the $x_j$ is done by setting these variables to $\infty$ in the expression $\underset{j=1}{\overset{d}{\Pi}}\varphi_{j}(v_{j}(\mathbf{x}))$. The marginal density can be obtained by taking derivatives of the marginal CDF. For a block-triangular matrix with block size $S$ this will generate no more than $Sd$ terms. Conditional PDFs and CDFs can be obtained from the marginals and the joints as before. 

% We can also include permutations to group the variables in different ways. 
% % In order to combine this approach with the HT decomposition of the tensor $A$, we simply set the permutation matrix $P$ to be an identity. This ensures that each summand in the expression $\left\langle A,\Phi(\mathbf{y})\right\rangle $ is a valid CDF.  
% }
% \subsection{A simple example}
% Consider the transformation 
% \eqan 
% v_1 &=& x_1
% \\
% v_2 &=& \alpha \sigma(x_1) + x_2
% \enan 
% We model the CDF of $(v_1,v_2)$ as
% \eqan 
% F(v_1,v_2) = \phi_{1}(v_1) \phi_2(v_2)
% \label{eq:CD\varphi_v}
% \enan
% and the pdfs is
% \eqan 
% p(x_1,x_2) &=& p(v_1,v_2) 
% \\
% &=&  \phi_{1}'(v_1) \phi_2'(v_2)
% \\
% &=& \phi_{1}'(x_1) \phi_2'(\alpha \sigma(x_1) + x_2)
% \label{eq:density_v}
% \enan 
% where we used that the 
% Jacobian is unity. 

% To obtain the marginal $p(x_2)$, we start 
% with the CFD
% \eqan 
% F(x_2, x_1=\infty) = \phi_2(\alpha +x_2),
% \enan 
% where we used (\ref{eq:CD\varphi_v}), 
% and take the derivative w.r.t. $x_2$,
% \eqan 
% p(x_2) = \phi_2'(\alpha +x_2)\,.
% \enan 
% To verify that this expression is consistent with (\ref{eq:density_v}), note that 
% \eqan 
% \int_{-\infty}^{+\infty}dx'_1 p(x'_1,x_2) &=& \int_{-\infty}^{+\infty}dx'_1\phi_{1}'(x'_1) \phi_2'(\alpha \sigma(x'_1) + x_2)
% \\
% &=& \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{+\infty}dx'_1
% \int_{-\infty}^{+x_2}dx'_2
% \phi_{1}'(x'_1) 
% \phi_2'(\alpha \sigma(x'_1) + x_2')
% \\
% &=&
% \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{+\infty}dv'_1
% \int_{-\infty}^{\alpha +x_2  }dv'_2
% \phi_{1}'(v'_1) 
% \phi_2'(v_2')
% \\
% &=&
% \int_{-\infty}^{+\infty}dv'_1
% \phi_{1}'(v'_1) 
% \, \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \\
% &=& \phi_2'(\alpha + x_2)
% \enan 

% \subsubsection*{Three variables}
% \eqan 
% p(x_1,x_2,x_3) &=& p(v_1,v_2,v_3) 
% \\
% &=&  \phi_{1}'(v_1) \phi_2'(v_2) \phi_3'(v_3)
% \\
% &=& \phi_{1}'(x_1) \phi_2'(\alpha \sigma(x_1) + x_2)
% \phi_3'(\alpha_{31} \sigma(x_1) + \alpha_{32} \sigma(x_2) + x_3)
% \label{eq:density_v3}
% \enan 
% where we used that the 
% Jacobian is unity. 

% % To obtain the marginal $p(x_2,x_3)$, we start 
% % with the CFD
% % \eqan 
% % F(x_2, x_1=\infty) = \phi_2(\alpha +x_2),
% % \enan 
% % where we used (\ref{eq:CD\varphi_v}), 
% % and take the derivative w.r.t. $x_2$,
% % \eqan 
% % p(x_2) = \phi_2'(\alpha +x_2)\,.
% % \enan 
% % To verify that this expression is consistent with (\ref{eq:density_v}), note that 
% {\tiny 
% \eqan 
% \int_{-\infty}^{+\infty}dx'_1 p(x'_1,x_2,x_3) &=&
% \int_{-\infty}^{+\infty}dx'_1
% \phi_{1}'(x_1') \phi_2'(\alpha \sigma(x_1') + x_2)
% \phi_3'(\alpha_{31} \sigma(x_1') + \alpha_{32} \sigma(x_2) + x_3)
% \nn 
% \\
% &=& \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{+\infty}dx'_1
% \int_{-\infty}^{+x_2}dx'_2
% \int_{-\infty}^{+x_3}dx'_3
% \phi_{1}'(x_1') \phi_2'(\alpha \sigma(x_1') + x_2')
% \phi_3'(\alpha_{31} \sigma(x_1') + \alpha_{32} \sigma(x_2') + x_3')
% \nn 
% \\
% &=&
% \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{+\infty}dv'_1
% \int_{-\infty}^{\alpha +x_2  }dv'_2
% \int_{-\infty}^{\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3 }dv'_3
% \phi_{1}'(v'_1) 
% \phi_2'(v_2')
% \phi_3'(v_3')
% \\
% &=&
% \int_{-\infty}^{+\infty}dv'_1
% \phi_{1}'(v'_1) 
% \, 
% \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \int_{-\infty}^{\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3 }dv'_3 \phi_3'(v_3')
% \\
% &=& 
% \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \phi_3'(\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3)
% \\
% &=& 
% \frac{\partial}{\partial x_2} 
% \left[ 
% \phi_2(\alpha + x_2)
% \phi_3'(\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3)
% \right]
% \enan 
% }


\subsection{MDMA sampling}

Given an MDMA as in \cref{eq:F_general_A}, we can sample in the same manner as for autoregressive models:
from $u_{1},\dots,u_{d}$ independent $U(0,1)$ variables, we obtain a sample from $F_{A,\Phi}$ by computing 
\begin{align*}
x_{1} =F_{A,\Phi}^{-1}(u_{1}),\quad x_{2} =F_{A,\Phi}^{-1}(u_{2}|x_1) \quad \cdots \quad x_{d} = F_{A,\Phi}^{-1}(u_{d}|x_{1},\dots,x_{d-1}),
\end{align*}
where, unlike with autoregressive model, the order of taking the conditionals does not need to be fixed.
The main drawback of this method is that due to the sequential nature of the sampling the computational cost is linear in $d$ and cannot be parallelized.

However, the structure of $F_{A,\Phi}$ can be leveraged to sample far more efficiently.
Define by $R_{A}$ a vector-valued categorical random variable taking values in $\left[m\right] \times \cdots \times \left[m\right]$, with distribution 
\begin{align*}
    \mathbb{P}\left[R_{A}=(i_{1},\dots,i_{d})\right]=A_{i_{1},\dots,i_{d}}.
\end{align*}
The fact that $A \in \Acal_{d,m}$ with $\Acal_{d,m}$ from \eqref{eq:define_acal} ensure the validity of this definition.
Consider a vector $(\tilde{X}_{1},\dots,\tilde{X}_{d},R_{A})$ where $R_A$ is distributed as above, and 
\begin{align*}
    \mathbb{P}\left[\tilde{X}_{1}\leq x_{1},\dots,\tilde{X}_{d}\leq x_{d}|R_{A}=\mathbf{r}\right]=\prod\limits_{i=1}^{d}\varphi_{r_{i},i}(x_{i}),
\end{align*}
for the collection $\{\varphi_{i,j}\}$ of univariate CDFs.
Denoting the distribution of this vector by $\tilde{F}_{A,\Phi}$, marginalizing over $R_A$ gives 
\begin{align*}
	\tilde{F}_{A,\Phi}(\bm x)=\underset{\mathbf{r}\in[m]^{d}}{\sum}\mathbb{P}\left[R_{A}=\mathbf{r}\right]\prod\limits_{j=1}^{d}\varphi_{r_{j},j}(x_{j})
	%=\underset{i_{1},\dots,i_{d}=1}{\overset{m}{\sum}}A_{i_{1},\dots,i_{d}}\prod\limits_{i=1}^{d}\varphi_{i_{j},j}(x_{j})
	=F_{A,\Phi}(\bm x).
\end{align*}
Instead of sampling directly from the distribution $F_{A,\Phi}$, we can thus sample from $\tilde{F}_{A,\Phi}$ and discard the sample of $R_A$.
To do this, we first sample from the categorical variable $R_A$. Denoting this sample by $\mathbf{r}$, we can sample from $\tilde{X}_{i}$ by inverting the univariate CDF $\varphi_{r_{i},i}$.
This can be \textit{parallelized} over $i$. 

The approach outlined above is impractical since $R_{A}$ can take $m^d$ possible values, yet if $A$ can be expressed by an efficient tensor representation this exponential dependence can be avoided. 
Consider the HT decomposition \cref{eq:HT}, which can be written as 
\begin{align}\label{eq:HT_mixture}
F_{A^{\mathrm{HT}},\Phi}(\bm{x})=\left\langle A^{\mathrm{HT}},\Phi(\bm{x})\right\rangle =\prod\limits _{\ell=1}^{p}\prod\limits _{j_{\ell}=1}^{2^{p-\ell}}\sum\limits _{k_{\ell,j_{\ell}}=1}^{m}\lambda_{k_{\ell+1,\left\lceil j_{\ell}/2\right\rceil },k_{\ell,j_{\ell}},j_{\ell}}^{\ell}\Phi(\bm{x})_{k_{1,1},\dots,k_{1,d/2}},
\end{align}
that is a normalized sum of $O(md)$ univariate CDFs. 
\begin{proposition}\label{prop:HT_sampling}
Sampling from \eqref{eq:HT_mixture} can be achieved in $O(\log d)$ time requiring the storage of only $O(d)$ integers.
\end{proposition}
Note that the time complexity of this sampling procedure depends only logarithmically on $d$.
The reason is that a simple hierarchical structure of Algorithm \ref{algo:ht_sampling}, where $\textrm{Mult}$ denotes the multinomial distribution.
\begin{figure}[ht]
\vspace{-.2in}
  \centering
  \begin{minipage}{.7\linewidth}
  \begin{algorithm}[H]
    \SetAlgoLined
    \KwResult{$x_j$ for $j= 1, \dots, d$}
    $k_{p,1}  \sim \textrm{Mult}(\lambda_{*}^p)$\;
     \For{$\ell \gets p - 1$ \KwTo $1$ \KwBy $-1$}{
      $ k_{\ell,j} \sim \textrm{Mult}(\lambda^{\ell}_{k_{\ell + 1, \left\lceil j/2\right\rceil }, *,j}), \qquad j = 1, \dots, 2^{p - \ell}$\;
     }
     $ x_j \sim \varphi_{k_{1, \left\lceil j/2\right\rceil},j}, \qquad j=1, \dots, 2^{p}$\;
     \caption{Sampling from the HT MDMA}\label{algo:ht_sampling}
    \end{algorithm}
    \end{minipage}
    \vspace{-.2in}
    \label{alg:HT}
\end{figure}
% The reason is that a simple hierarchical algorithm for sampling is as follows:
% \begin{align*}
%     k_p & \sim \textrm{Mult}(\lambda_{*}^p) 
%     \\
%     k_{p-1,j} & \sim \textrm{Mult}(\lambda^{p-1}_{k_p, *,j}) && j=1,2
%     \\
%     k_{p-2,j} & \sim \textrm{Mult}(\lambda^{p-2}_{k_{p-1, j/2  }, *,j}) && j=1,2,3,4
%     \\
%     \vdots
%     \\
%     k_{1,j} & \sim \textrm{Mult}(\lambda^{1}_{k_{2,  j/2  }, *,j}) && j=1, \dots, 2^{p-1}
%     \\
%     x_j & \sim \varphi_{k_{1, j/2},j}  && j=1, \dots, 2^{p},
% \end{align*}

% \begin{algorithm}[H] 
% \caption{Sampling from the HT MDMA}\label{algo:ht_sampling}
% \begin{algorithmic}
% \STATE  $k_p  \sim \textrm{Mult}(\lambda_{*}^p)$
% \FOR{$\ell=1$ {\bfseries to} $p - 1$}
% \STATE 
% $ k_{p-\ell,j} \sim \textrm{Mult}(\lambda^{p-\ell}_{k_p - \ell + 1, *,j}), \qquad j = 1, \dots, 2^{\ell}$
% \ENDFOR
% \STATE $ x_j \sim \varphi_{k_{1, j/2},j}, \qquad j=1, \dots, 2^{p}$
% \STATE {\bfseries Output:} $ x_j, \qquad j=1, \dots, 2^{p}$
% \end{algorithmic}
% \end{algorithm}
% % \end{minipage}
The logarithmic dependence is only in the sampling from the categorical variables, which is inexpensive to begin with.
We thus avoid the linear dependence of the time complexity on $d$ that is common in sampling from autoregressive models. Furthermore, the additional memory required for sampling scales like $\log m$ (since storing the categorical samples requires representing integers up to size $m$), and aside from this each sample requires evaluating a single product of univariate CDFs (which is independent of $m$). In preliminary experiments, we have found that even for densities with $d \leq 10$, this sampling scheme is faster by $1.5$ to $2$ orders of magnitude than autoregressive sampling. The relative speedup should only increase with $d$. 







==> Marginalizable Density Models (4)/arxiv/proofs.tex <==
%!TEX root = ../MDN_neurips.tex

\section{Proofs} \label{app:proofs}

\subsection{Proof of \Cref{prop:HT_sampling}}

The proof follows directly from Algorithm \ref{algo:ht_sampling}. The distribution $F_{A^{\mathrm{HT}},\Phi})=\left\langle A^{\mathrm{HT}},\Phi\right\rangle$ is a mixture model, and thus in order to sample from it we can first draw a single mixture component (which is a product of univariate CDFs) and then sample from this single component. The mixture weights are the elements of the tensor $A^{\mathrm{HT}}$ given by the diagonal HT decomposition \cref{eq:HT_mixture}. In the next section, we add details on the sampling process for the sake of clarity.

\subsubsection{Details on the sampling for the HT model}
Define a collection of independent categorical variables $R=\{R^\ell_{i,j}\}$ taking values in $[m]$, where $\ell \in [p], i \in [m]$ and for any $\ell$, $j \in [2^{p-\ell}]$. These variables are distributed according to  
\begin{align*}
	\forall\ell,i,j:\quad\mathbb{P}\left[R_{i,j}^{\ell}=k\right]=\lambda_{i,k,j}^{\ell},
\end{align*}
where $\{ \lambda^{\ell} \}_{\ell=1}^{p}$ are the parameters of the HT decomposition. The fact that the parameters are nonnegative and $\sum_{k=1}^m \lambda_{k,i,j}^{\ell} = 1$ ensures the validity of this distribution.

With the convention $R_{k_{p+1,1},1}^{p}=R_{1,1}^{p}$, define the event
\begin{align*}
\underset{\ell=1}{\overset{p}{\bigcap}}\left(\cap_{j_{\ell}=1}^{2^{p-\ell}}\left\{ R_{k_{\ell+1,\left\lceil j_{\ell}/2\right\rceil },j_{\ell}}^{\ell}=k_{\ell,j_{\ell}}\right\} \right) &=
    \left\{ R_{1,1}^{p}=k_{p,1}\right\} \\
&\phantom{=}\bigcap\left(\cap_{j=1}^{2}\left\{ R_{k_{p,1},j}^{p-1}=k_{p-1,j}\right\} \right)\\
&\phantom{=}\,\,\,\,\vdots\\
&\phantom{=}\bigcap\left(\cap_{j=1}^{d/2}\left\{ R_{k_{2,\left\lceil j/2\right\rceil },j}^{1}=k_{1,j}\right\} \right).
\end{align*}
Let $(\tilde{X}_{1},\dots,\tilde{X}_{d}, R)$ be a random vector such that
\begin{align} \label{eq:sample_HT}
% \mathbb{P}\left[\tilde{X}_{1}\leq x_{1},\dots,\tilde{X}_{d}\leq x_{d}| \cap_{\ell=1}^p \{R^{\ell}=\mathbf{k}^{\ell}\}\right]=\prod_{i=1}^{d}\varphi_{k_{1,i/2},i}(x_{i}),
\mathbb{P}\left[\tilde{X}_{1}\leq x_{1},\dots,\tilde{X}_{d}\leq x_{d}\left|\underset{\ell=1}{\overset{p}{\bigcap}}\left(\cap_{j_{\ell}=1}^{2^{p-\ell}}\left\{ R_{k_{\ell+1,\left\lceil j_{\ell}/2\right\rceil },j_{\ell}}^{\ell}=k_{\ell,j_{\ell}}\right\} \right)\right.\right] 
= \prod_{i=1}^{d}\varphi_{k_{1,\left\lceil i/2\right\rceil },i}(x_{i}),
\end{align}
which implies that the distribution of $(\tilde{X}_{1},\dots,\tilde{X}_{d})$ obtained after conditioning on a subset of the $\{R^\ell_{i,j}\}$ in this way is equal to a single mixture component in $F_{\mathrm{HT}}=\left\langle A,\Phi\right\rangle$.
Thus, based on a sample of $R$, one can sample $\tilde{X}_{i}$ by inverting the univariate CDFs $\varphi_{k_{1,\left\lceil i/2\right\rceil },i}$ numerically and parallelizing over $i$. 
Numerical inversion is trivial since the functions are increasing and continuously differentiable, and this can be done for instance using the bisection method.
It remains to sample a mixture component.

Assume that a sample $\{R_{i,j}^{\ell}\}$ for a sequence of variables as in \cref{eq:sample_HT} is obtained e.g. from Algorithm \ref{algo:ht_sampling}.
With the convention $\lambda_{k_{p+1,1},k,1}^{p}=\lambda_{k}^{p}$, since 
\begin{align*}
% 	\mathbb{P}\left[ R^{p}_{1,1}=k_{p}\cap R_{k_{p},1}^{p-1}=k_{p-1,1}\cap R_{k_{p},2}^{p-1}=k_{p-1,2},\dots,R_{k_{2,d/2},d/2}^{1}=k_{1,d/2}\right]= 
% 	\prod\limits_{\ell=1}^p \prod\limits_{j_{\ell}=1}^{2^{p - \ell + 1}} \lambda_{k_{\ell,j_{\ell}},k_{\ell-1, j_{\ell}/2 },j_{\ell}}^{\ell},
\mathbb{P}\left[\underset{\ell=1}{\overset{p}{\bigcap}}\left(\cap_{j_{\ell}=1}^{2^{p-\ell}}\left\{ R_{k_{\ell+1,\left\lceil j_{\ell}/2\right\rceil },j_{\ell}}^{\ell}=k_{\ell,j_{\ell}}\right\} \right)\right]=\prod\limits _{\ell=1}^{p}\prod\limits _{j_{\ell}=1}^{2^{p-\ell}}\lambda_{k_{\ell+1,\left\lceil j_{\ell}/2\right\rceil },k_{\ell,j_{\ell}},j_{\ell}}^{\ell},
\end{align*}
sampling from the categorical variables in this fashion is equivalent to sampling a mixture component.
It follows that by first sampling a single mixture component and then sampling from this component, one obtains a sample from $F_{\mathrm{HT}}$. 

The main loop in Algorithm \ref{algo:ht_sampling} samples such a mixture component, and there are $p= \log_2 d $ layers in the decomposition, so the time complexity of the main loop is $O(\log d)$, and aside from storing the decomposition itself this sampling procedure requires storing only $O(d)$ integers. This logarithmic dependence is only in sampling from the categorical variables which is computationally cheap. This not only avoids the linear time complexity common in sampling from autoregressive models (without using distillation), but the space complexity is also essentially independent of $m$ since only a single mixture component is evaluated per sample. 

%Thus, one can sample from $(\tilde{X}_{1},\dots,\tilde{X}_{d},\{R_{i,j}^{\ell}\})$ instead.

% Sampling $\{R_{i,j}^{\ell}\}$ is best done sequentially starting from the final layer:
% \begin{enumerate}
%     \item Sample from $R^{p}_{1,1}$ to obtain a sample $k_{p}$.
%     \item Sample from $R_{k_{p},1}^{p-1},R_{k_{p},2}^{p-1}$ to obtain samples $k_{p-1,1},k_{p-1,2}$.
%     \item Proceed similarly until the reaching the first layer.
% \end{enumerate}
 %\bigcap_{j=1}^{} 

%\newpage
\subsection{Proof of \Cref{prop:universal_1}}

% \begin{definition}
% $\Gcal = \{g\colon \R^d \to \R \}$ is dense in $\Fcal = \{g\colon \R^d \to \R \}$ with respect to the uniform norm if, for any $f \in \Fcal$, compact $K \subset \R^d$, and $\epsilon \ge 0$, there exists $g \in \Gcal$ such that
% \begin{align*}
%   \| f - g \|_{\infty,K} = \sup_{x \in K} |g(x) - f(x) | \le \epsilon.
% \end{align*}
% \end{definition}

% \Cref{prop:universal_1} follows from \Cref{prop:universal_1b} and the fact that $\cup_l \Phi_{l,r,\sigma} \subseteq \cup_{l,r} \Phi_{l,r,\sigma}$.

% \begin{proposition}\label{prop:universal_1b}
% $\cup_l \Phi_{l,r,\sigma}$ is dense in $\Fcal_1$ with respect to the uniform norm for any $w \ge 4$.
% \end{proposition}
Assume that the activation function $\sigma$ is increasing, continuously differentiable, and such that $\lim_{x\to-\infty}\sigma(x) = 0$ and $\lim_{x\to\infty} \sigma(x) = 1$.
\Cref{prop:universal_1} then follows immediately from \Cref{prop:universal_1a} and the fact that $\cup_r \Phi_{1,r,\sigma} \subseteq \cup_{l,r} \Phi_{l,r,\sigma}$.
\begin{remark}
    In practice, we use the activation $\sigma(x) = x + a \tanh(x)$ for some $a > -1$.
    While it does not satisfy the assumptions, the arguments in the proof of \Cref{prop:universal_1b} can be modified in a straightforward manner to cover this activation (see \Cref{rmk:activation_cdf}).
\end{remark}
\begin{proposition}\label{prop:universal_1a}
$\cup_r \Phi_{1,r,\sigma}$ is dense in $\Fcal_1$ with respect to the uniform norm.
\end{proposition}
Letting
\begin{align*}
 \widetilde{\Fcal}_1 &= \{\widetilde{F}\colon \R \to \R,\, \widetilde{F}(x) = \log F(x)/(1-F(x)),\, F \in \Fcal_1\},\\
\widetilde{\Phi}_{l,r,\sigma} &= \{\widetilde{\varphi} \colon \R \to \R,\, \widetilde{\varphi}(x) = \log \varphi(x)/(1-\varphi(x)),\,\varphi \in \Phi_{l,r,\sigma}\},
\end{align*}
the proof of \Cref{prop:universal_1a} relies on the following proposition.
% \begin{proposition}\label{prop:universal_1b}
% $\cup_r \widetilde{\Phi}_{1,r,\sigma}$ is dense in $\widetilde{\Fcal}_1$ with respect to the uniform norm.
% \end{proposition}
\begin{proposition}\label{prop:universal_1b}
$\cup_r \widetilde{\Phi}_{1,r,\sigma}$ is dense in $\widetilde{\Fcal}_1$ with respect to the uniform norm.
\end{proposition}


\subsubsection{Proof of \Cref{prop:universal_1a}}
This proof is similar to that of \cite[][Theorem 2]{dugas2009incorporating}, which deals with functions with positive outputs.
We want to show that, for any $F \in \Fcal_1$, compact $K \subset \R$, and $\epsilon > 0$, there exists $\varphi \in \cup_r \Phi_{1,r,\sigma}$ such that
\begin{align*}
     \| \varphi - F \|_{\infty,K}   = \sup_{x \in K} |\varphi(x) - F(x) | \le \epsilon.
\end{align*}

Denote the sigmoid function by $\rho(x) = 1/(1 + e^{-x})$ and define the function $\widetilde{F}\colon \R \to \R$ by $\widetilde{F}(x) = \log F(x)/(1-F(x))$, so that $F = \rho \circ \widetilde{F}$.
% Let $\widetilde{\Phi}_{l,r,\sigma}$ denote the class of unconstrained feedborward neural networks that have the same architecture as $\Phi_{l,r,\sigma}$, that is
% \begin{align*}
% \widetilde{\Phi}_{l,r,\sigma} = \{\widetilde{\varphi} \colon \R \to \R, \widetilde{\varphi}(x) = L_{l} \circ \sigma \circ L_{l-1} \circ \sigma \cdots \circ \sigma \circ L_1 \circ \sigma \circ L_0(x)\},
% \end{align*}
% where $L_i \colon \R^{n_{i}} \to \R^{n_{i+l}}$ is the affine map $L_i(x) = W_i x + b_i$ for an $n_{i+1} \times n_{i}$ weight matrix $W_i$ and an $n_{i+1} \times 1$ bias vector $b_i$, with $n_{l+1} = n_0 = 1$ and $n_i = w$ for $i \in [l]$.
% By \citep[][Theorem 3.2]{kidger2020}, for every $\epsilon \ge 0$, there exists $ \widetilde{\varphi} \in \cup_{l} \widetilde{\Phi}_{l,4,\sigma}$ such that
% \begin{align*}
% \sup_{x \in K} |\widetilde{\varphi}(x) - \widetilde{F}(x)| \le \epsilon.
% \end{align*}
% Thus, letting $\varphi = \rho \circ \widetilde{\varphi}$, we have
% \begin{align*}
%     |\varphi(x) - F(x)|  = |\rho \circ \widetilde{\varphi}(x) - \rho \circ \widetilde{F}(x)|   \le \sup_{x \in K}\rho(x)'|\widetilde{\varphi}(x) - \widetilde{F}(x)|   \le \frac{\epsilon}{4}.
% \end{align*}
% Since $\Phi_{l,r,\sigma} = \{\rho \circ \widetilde{\varphi}\colon \widetilde{\varphi} \in  \widetilde{\Phi}_{l,r,\sigma}{\color{red}, W_i \ge 0\,\, \forall i}\}$, the result follows.
%\cite{dugas2009incorporating}
By \Cref{prop:universal_1b},
there exists $ \widetilde{\varphi} \in \cup_{r} \widetilde{\Phi}_{1,r,\sigma}$ such that
\begin{align*}
\sup_{x \in K} |\widetilde{\varphi}(x) - \widetilde{F}(x)| \le 4 \epsilon.
\end{align*}
Thus, letting $\varphi = \rho \circ \widetilde{\varphi}$, we have
\begin{align*}
    |\varphi(x) - F(x)|  = |\rho \circ \widetilde{\varphi}(x) - \rho \circ \widetilde{F}(x)|   \le \sup_{x \in K}\rho(x)'|\widetilde{\varphi}(x) - \widetilde{F}(x)|   \le \epsilon.
\end{align*}
Since $\Phi_{1,r,\sigma} = \{\rho \circ \widetilde{\varphi}\colon \widetilde{\varphi} \in  \widetilde{\Phi}_{1,r,\sigma}\}$, the result follows.

\subsubsection{Proof of \Cref{prop:universal_1b}}
This proof is similar to that of \cite[][Theorem 3.1]{Daniels2010}, which is incomplete and only deals with the sigmoid activation.
First, note that $ \widetilde{\Fcal}_1$ is the space of strictly increasing and continuously differentiable functions.
Therefore, for any $\widetilde{F} \in \widetilde{\Fcal}_1 $ and interval $K = [K_1, K_2]$, we can write, for any $x \in K$,
\begin{align*}
    \widetilde{F}(x) 
    =\widetilde{F}(K_1) + \int_{\widetilde{F}(K_1)}^{\widetilde{F}(K_2)} \Ind_{\widetilde{F}(x) \ge u} du =\widetilde{F}(K_1) + \int_{\widetilde{F}(K_1)}^{\widetilde{F}(K_2)} \Ind_{x \ge \widetilde{F}^{-1}(u)}du,
\end{align*}
where the existence of the inverse $\widetilde{F}^{-1}$ is guaranteed by the fact that $\widetilde{F}$ is strictly increasing and continuous.
Thus, for $\widetilde{F}(K_1) = u_0 < u_1 < \cdots < u_k = \widetilde{F}(K_2)$ a partition of $[\widetilde{F}(K_1),\widetilde{F}(K_2)]$ with $u_{j+1} - u_j \le \epsilon /2(\widetilde{F}(K_2) - \widetilde{F}(K_1))$, $x_j = \widetilde{F}^{-1}(u_j)$ and
\begin{align*}
  G(x) = \widetilde{F}(K_1) + \sum_{j=1}^k \Ind_{x \ge x_j} (u_{j} - u_{j-1}),
\end{align*}
we have $| \widetilde{F}(x) - G(x)| \le \epsilon/2$, namely the approximation error of the Riemann sum for increasing functions.
Let $a > 0$ and $\widetilde{\varphi} \in \widetilde{\Phi}_{1,k,\sigma}$ obtained by setting $b_1 =  \widetilde{F}(K_1)$, as well as $(W_1)_{1,j} = (u_{j} - u_{j-1})/a > 0$, $(b_{0})_j =-ax_j$ and $(W_0)_{j,1} = a$ for $1 \le j \le k$, then
\begin{align*}
   |G(x) - \widetilde{\varphi}(x)| \le \sum_{j=1}^k (u_{j+1} - u_j) \left|\Ind_{x \ge x_j} - \sigma(a(x - x_j))\right|.
\end{align*}
By the assumptions on $\sigma$, it is clear that $|\Ind_{x\ge0} - \sigma(ax)|$ can be made arbitrarily small.
Thus, taking $a$ large enough so that $  |G(x) - \widetilde{\varphi}(x)| \le \epsilon/2$, we have
\begin{align*}
    | \widetilde{F}(x) - \widetilde{\varphi}(x)| \le | \widetilde{F}(x) - G(x)| +|G(x) - \widetilde{\varphi}(x)| \le  \epsilon.
\end{align*}

\begin{remark}\label{rmk:activation_cdf}
   Let $\sigma(x) = x + a \tanh(x)$ for some $a > -1$ and $\widetilde{\varphi} \in \widetilde{\Phi}_{1,k,\sigma}$ obtained by setting $b_1 =  \widetilde{F}(K_1) + 1/2$, as well as $(W_1)_{1,j} = (u_{j} - u_{j-1})/2a > 0$, $(b_{0})_j =-ax_j$ and $(W_0)_{j,1} = |a|$ for $1 \le j \le k$, then
\begin{align*}
   |G(x) - \widetilde{\varphi}(x)| 
   &\le\sum_{j=1}^k (u_{j+1} - u_j) \left|\Ind_{x \ge x_j} - \tanh(|a|(x - x_j))/2 - 1/2\right| \\
   &\phantom{=}+  \sum_{j=1}^k (u_{j+1} - u_j) |x - x_j|/2|a|.
\end{align*}
Because $a$ is arbitrary, one can take it large enough so that  $  |G(x) - \widetilde{\varphi}(x)| \le \epsilon/2$ as above.
\end{remark}

% \begin{proposition}
% Let $F\colon \R \to \R$ be a strictly increasing and continuous function.
% Then, for every $\epsilon > 0$, there exists a partition $\infty = x_0 < x_1 < \cdots < x_k = \infty$  of $\R$ such that the piecewise constant function $G(x) = \sum_{j=1}^{k} F(x_{j-1}) \Ind_{x \in [x_{j-1},x_j)}$ satisfies $\|F - G\|_{\infty} \le \epsilon$.
% \end{proposition}
% \begin{proof}
%     For $1 \le j \le k - 1$, let
%     \begin{align*}
%         x_{j+1} = \sup\{x\colon F(x) \le F(x_j)\},
%     \end{align*}
%     leading to $\max_{1 \le j \le k} F(x_{j}) - F(x_{j-1}) \le \epsilon$, 
%     and thus
%     \begin{align*}
%         \|F - G\|_{\infty} =  \max_{1 \le j \le k} F(x) - F(x_{j-1}) \le \epsilon. 
%     \end{align*}
% \end{proof}

\subsection{Proof of \Cref{prop:universal_d}}

% \begin{remark}
%     In \Cref{sec:multivariate,sec:theory} from an earlier version of the manuscript, a typo mention defines the support and image of $\bm \Phi$ as $\R^d$ and $[0,1]^{m}\times \cdots \times [0,1]^m$ instead of $\R^d \times [m]^d$ and $[0,1]$.
% \end{remark}
Consider the classes of order $d$ tensored-valued functions with $m$ dimensions per mode defined as
\begin{align*}
    \Phi_{m,d,l,r,\sigma} &= \{ \Phi \colon \R^d \times [m]^d \to [0,1], \, \Phi(\bm x)_{i_1, \dots, i_d} = \textstyle \prod\limits_{j=1}^{d}\varphi_{i_{j},j}(x_{j}),\, \varphi_{i,j} \in \Phi_{l,r,\sigma}\}, \\
    \Fcal_{m,d} &= \{ \Phi \colon \R^d \times [m]^d \to [0,1], \, \Phi(\bm x)_{i_1, \dots, i_d} = \textstyle \prod\limits_{j=1}^{d}F_{i_{j},j}(x_{j}),\, F_{i,j} \in \Fcal_1 \}
\end{align*}
as well as the class of neural network-based and $\Fcal_1$-based MDMAs, that is
\begin{align*}
    \textrm{MDMA}_{m,d,l,r,\sigma} &= \{ F_{A,\Phi}\colon\R^d \to [0,1],\,F_{A,\Phi}(\bm x)= \langle A, \Phi(\bm x) \rangle, \, A \in \Acal_{d,m},\, \Phi \in  \Phi_{m,d,l,r,\sigma} \}, \\
 \textrm{MDMA}_{m,d,\Fcal_1} &=  \{F_{A,\Phi} \colon\R^d \to [0,1],\, F_{A,\Phi}(\bm x)= \langle A, \Phi(\bm x) \rangle, \, A \in \Acal_{d,m},\, \Phi \in  \Fcal_{m,d}\}.
\end{align*}
We can now state the following proposition.
\begin{proposition}\label{prop:universal_da}
$\cup_{l,r} \mathrm{MDMA}_{m,d,l,r,\sigma}$ is dense in $ \mathrm{MDMA}_{m,d,\Fcal_1}$ with respect to the uniform norm
\end{proposition}
\Cref{prop:universal_d} then follows immediately from the fact that $\cup_{m} \textrm{MDMA}_{m,d,\Fcal_1}$ is the space of multivariate mixture distributions admitting a density, which is dense in $\Fcal_d$ with respect to the uniform norm (see e.g.,  \cite[][Theorem 33.2]{DasGupta2008}, \cite[][Theorem 5]{Cheney2009}, or \cite[][Corollary
11]{Nguyen2019}).

\subsubsection{Proof of \Cref{prop:universal_da}}

With $A \in \Acal_{d,m}$, $\Phi_1 \in \Phi_{m,d,l,r,\sigma}$,  and $\epsilon > 0$ and a compact $K = K_1 \times \cdots \times K_d \subset \R^d$, we want to prove that there exists
$A_2 \in \Acal_{d,m}$ and $\Phi_2 \in \Fcal_{m,d}$, such that $\sup_{\bm x \in K} |F_{A,\Phi_1}(\bm x) - F_{A_2,\Phi_2}(\bm x)| \le \epsilon$.
Assuming that we can show $\sup_{\bm x \in K} |\Phi_1(\bm x)_{i_1,\dots,i_d}-  \Phi_2(\bm x)_{i_1,\dots,i_d}| \le \epsilon$, the result would then follow from setting $A_2 = A$ and the fact that $F_{A,\Phi_1}(\bm x) - F_{A,\Phi_2}(\bm x) = \langle A, \Phi_1(\bm x) -  \Phi_2(\bm x) \rangle $ implies
\begin{align*}
    \sup_{\bm x \in K} | F_{A,\Phi_1}(\bm x) - F_{A,\Phi_2}(\bm x) | = 
    %&=\sup_{\bm x \in K} | \langle A, \Phi_1(\bm x) -  \Phi_2(\bm x)  \rangle | \\
    &\le \sum_{i_1,\dots,i_d} A_{i_1,\dots,i_d} \sup_{\bm x \in K} |\Phi_1(\bm x)_{i_1,\dots,i_d}-  \Phi_2(\bm x)_{i_1,\dots,i_d}|
    = \epsilon.
\end{align*}
% The result then follows immediately from \Cref{prop:universal_1} and the fact that $\cup_{m} \textrm{MDMA}_{m,d,\Fcal_1}$ is the space of multivariate mixture distributions, which is dense in $\Fcal_d$ with respect to the uniform norm.

With $\delta = \epsilon^{1/d}$, by \Cref{prop:universal_1}, there exists $l$, $w$, and $\{\varphi\}_{i \in [m],j \in [d]}$ with $\varphi_{i,j} \in  \Phi_{l,r,\sigma}$, such that
\begin{align*}
    \max_{i \in [m],j \in [d]} \sup_{x_j \in K_j}|\varphi_{i,j}(x_j) - F_{i,j}(x_j)| \le \delta.
\end{align*}
Thus, we have that
\begin{align*}
   |\Phi_1(\bm x)_{i_1,\dots,i_d}-  \Phi_2(\bm x)_{i_1,\dots,i_d}| = 
    | \prod\limits_{j=1}^{d}\varphi_{i_j,j}(x_{j}) - \prod_{j=1}^d F_{i,j}(x_j)| \le \delta^d = \epsilon.
\end{align*}


==> Marginalizable Density Models (4)/arxiv/sampling.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Sampling}
\begin{align*}
\begin{aligned}
    k_p & \sim \textrm{Mult}(\lambda_{*}^p)
    \\
    k_{p-1,j} & \sim \textrm{Mult}(\lambda^{p-1}_{k_p, *,j}) & j=1,2
    \\
    k_{p-2,j} & \sim \textrm{Mult}(\lambda^{p-2}_{k_{p-1, j/2  }, *,j}) & j=1,2,3,4
    \\
    \vdots
    \\
    k_{1,j} & \sim \textrm{Mult}(\lambda^{1}_{k_{2,  j/2  }, *,j}) & j=1 \ldots 2^{p-1}
    \\
    x_j & \sim \varphi_{k_{1, j/2   },j}(x_j)  & j=1 \ldots 2^{p}
\end{aligned}
\end{align*}

==> Marginalizable Density Models (4)/arxiv/theory.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Universality of the MDMA}
\label{sec:theory}

To model functions in $\Fcal_1$, we use $\Phi_{l,r,\sigma}$, a class of constrained feedforward neural networks proposed in \cite{balle2018variational} with $l$ hidden layers, each with $r$ neurons, and $\sigma$ a nonaffine, increasing and continuously differentiable elementwise activation function, defined as
\begin{align*}
    \Phi_{l,r,\sigma} = \{ \varphi \colon \R \to [0,1],\, \varphi(x) = \mbox{sigmoid} \circ L_{l} \circ \sigma \circ L_{l-1} \circ \sigma \cdots \circ \sigma \circ L_1 \circ \sigma \circ L_0(x)\},
\end{align*}
where $L_i \colon \R^{n_{i}} \to \R^{n_{i+l}}$ is the affine map $L_i(x) = W_i x + b_i$ for an $n_{i+1} \times n_{i}$ weight matrix $W_i$ with \emph{nonnegative} elements and an $n_{i+1} \times 1$ bias vector $b_i$, with $n_{l+1} = n_0 = 1$ and $n_i = r$ for $i \in [l]$.
The constraints on the weights and the final sigmoid guarantee that $ \Phi_{l,r,\sigma} \subseteq \Fcal_1$, and for any $\varphi \in \Phi_{l,r,\sigma}$, the corresponding density $\varphid (x) = \partial \varphi(x) / \partial x$ can be obtained with the chain rule.
The universal approximation property of the class $\Phi_{l,r,\sigma}$ is expressed in the following proposition.
\begin{proposition}\label{prop:universal_1}
$\cup_{l,r} \Phi_{l,r,\sigma}$ is dense in $\Fcal_1$ with respect to the uniform norm.
\end{proposition}
While the proof in the supplementary assumes that $\lim_{x\to-\infty}\sigma(x) = 0$ and $\lim_{x\to\infty} \sigma(x) = 1$, it can be easily modified to cover other activations.
For instance, in our experiments, we use $\sigma(x) = x + a \tanh(x)$ following \cite{balle2018variational}, and refer to the supplementary material for more details regarding this case.
In the multivariate case, consider the class of order $d$ tensored-valued functions with $m$ dimensions per mode defined as
\begin{align*}
    \Phi_{m,d,l,r,\sigma} = \{ \Phi \colon \R^d \times [m]^d \to [0,1], \, \Phi(\bm x)_{i_1, \dots, i_d} = \textstyle \prod\limits_{j=1}^{d}\varphi_{i_{j},j}(x_{j}),\, \varphi_{i,j} \in \Phi_{l,r,\sigma}\}.
\end{align*}
Combining $\Phi_{m,d,l,r,\sigma}$ with the $\Acal_{d,m}$, the normalized tensors introduced in \Cref{sec:multivariate}, the class of neural network-based MDMAs can then be expressed as
\begin{align*}
    \textrm{MDMA}_{m,d,l,r,\sigma} = \{ F_{A,\Phi}\colon\R^d \to [0,1],\,F_{A,\Phi}(\bm x)= \langle A, \Phi(\bm x) \rangle, \, A \in \Acal_{d,m},\, \Phi \in  \Phi_{m,d,l,r,\sigma} \}.
\end{align*}
\begin{proposition}\label{prop:universal_d}
The set $\cup_{m,l,r} \textrm{MDMA}_{m,d,l,r,\sigma}$ is dense in $\Fcal_{d}$ with respect to the uniform norm.
\end{proposition}
The proof relies on the fact that setting $m=1$ yields a class that is dense in the space of $d$-dimensional CDFs with independent components. All proofs are provided in \Cref{app:proofs}. 

% \subsection{Bounding the generalization risk}

% Let $F_0 \in \Fcal_d$ be the true but unknown data-generating distribution and $X_1, \cdots, X_n$ an i.i.d. sample with $X_i \in \Xcal \subseteq \R^d \sim F_0$.
% For any $F \in \Fcal_d$ with corresponding density $f$, using the negative log-likelihood as loss function, the population risk for is $R(F) = R(f) = \E_{F_0} \log f(X)$, which is uniquely minimized at $F_0$, and the empirical risk is $R_n(F) = R_n(f) = -1/n \sum_{i=1}^n \log f(X_i)$.
% \begin{proposition}
% For every $\epsilon$ and $\delta \in (0,1)$, then $\sup_{F \in \Phi_{m,d,l,r,\sigma}} |R_n(F) - R(F)| \le \epsilon$ holds with probability at least $1 - \delta$ for $n$ sufficiently large.
% \end{proposition}
% In other words, the empirical risk can be used as a estimate of the population risk.
% {\color{red} Of course, the caveat is that ``sufficiently large'' is unknown.
% Depending on how much effort, we can make the bound fairly tight, but is it worth it or should I stick to something simple?}

% \subsubsection{Covering numbers}

% % For $X_1, \dots, X_n$ random elements in $(\Xcal, \Omega)$ with law $P$
% % and a measurable function $f: \Xcal  \to \R$, denote the \emph{expectation}, \emph{empirical measure} and \emph{empirical process} at $f$ respectively by
% % \begin{align*}
% %     P f = \int f(x)dP(x),
% %     \qquad \eP f = \frac{1}{n} \sum^n_{i=1} f(X_i), 
% %     \qquad \eG f= \sqrt{n}(\eP f - P f), 
% % \end{align*}
% % as well as $\|f\|_{L_r(P)} = \left\{\int \vert f(x)\vert^r dP(x)\right\}^{1/r}$ for the \emph{$L_r(P)$ norm}.

% Let $\Fcal$ be an arbitrary class of functions such that $(\Fcal, \|\cdot \|)$ is a subset of a normed space for some norm $\| \cdot \|$.
% A function $F$ is called an \emph{envelope} of $\Fcal$ if $F \ge \sup_{f \in \Fcal}| f |$. 
% Define $N(\epsilon, \Fcal, \|\cdot \|)$ as the \emph{covering number} of $\Fcal$,
% that is the minimum number of $\epsilon$-balls needed to cover $\Fcal$
% \begin{align*}
%     N(\epsilon, \Fcal, \|\cdot \|) = \inf \{N\colon \exists f_1, \dots, f_N \in \Fcal, \mbox{ s.t. } \Fcal \subset \cup_{i=1}^N B(f_k, \epsilon) \},
% \end{align*}
% where $B(f, \epsilon) = \{g \in \Fcal \colon \|f - g \| \le \epsilon \}$.
% $N(\epsilon, \Fcal, \|\cdot \|)$ measures the complexity of $\Fcal$: the larger the covering number, the larger the class.
% % The quantity $\log N(\epsilon, \Fcal, \|\cdot \|)$ is called the \emph{metric entropy}, and 
% % \begin{align*}
% %     J(\delta, \Fcal, \|\cdot \|_{L_2(Q)}) = \int_0^1 \sqrt{\sup_{Q} \log N(\epsilon \|F\|_{L_2(Q)}, \Fcal, \|\cdot \|_{L_2(Q)})} d\epsilon
% % \end{align*}
% % is called the \emph{uniform entropy integral}.

% Our first result concerns the classes that we use to model CDFs.
% \begin{proposition}
% With $d \ge 2$, there exist universal constants $c_1, c_2(d) < \infty$ such that, for $0 < \epsilon < 1$,
% \begin{align*}
%     \sup_{Q} \log N(\epsilon, \Phi_{l,r,\sigma}, \|\cdot \|_{L_2(Q)}) &\le c_1 \epsilon^{-1}, \\
%     \sup_{Q} \log N(\epsilon, \Phi_{d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}) &\le  c_2(d) \epsilon^{-1} [\log(1/\epsilon)]^{d - 1/2}, \\
%     \sup_{Q} \log N(\epsilon, \Phi_{m,d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}) &\le c_2(d) \epsilon^{-1} [\log(1/\epsilon)]^{d - 1/2}.
% \end{align*}
% \end{proposition}
% The universality of $c_1, c_2$ with respect to the architecture of the univariate networks or of the mixing tensors is a direct consequence of the fact that a shape constraint (i.e., monotonicity) simplifies considerably any function class.
% Note that the log factor is an artifact of the proof, which uses the fact that the classes we consider are subsets of $\Fcal_d$, but this could be improved to $c_2(d) \epsilon^{-1}$. 
% {\color{red} If interested, an alternative proof for $\Phi_{d,l,r,\sigma}$ is provided below, and something similar can be done for $\Phi_{m,d,l,r,\sigma}$.}
% % \begin{proof}
% % Since $\Phi_{l,r,\sigma} \subset \Fcal_1$ and $\Phi_{d,l,r,\sigma} \subset \Phi_{m,d,l,r,\sigma} \subset \Fcal_d$, we have
% % \begin{align*}
% %     N(\epsilon, \Phi_{l,r,\sigma}, \|\cdot \|_{L_2(Q)}) &\le N(\epsilon, \Fcal_1, \|\cdot \|_{L_2(Q)}),\\
% %     N(\epsilon, \Phi_{d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}) &\le N(\epsilon, \Phi_{m,d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}), \\
% %      N(\epsilon, \Phi_{m,d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}) &\le N(\epsilon, \Fcal_{d}, \|\cdot \|_{L_2(Q)}).
% % \end{align*}
% % The result follows from bounding the covering numbers of $\Fcal_1$ and $\Fcal_d$, using respectively  Theorem 2.7.5 from \cite{vanderVaart1996} and  Theorem 1.1 from \cite{blei2007}.
% % \end{proof}
% % The use bracketing numbers because it's convenient for product classes.
% % By Lemma 9.18 of \cite{kosorok2007}, we have
% % \begin{align*}
% %     N(\epsilon, \Phi_{d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}) \le N_{[]}(\epsilon, \Phi_{d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}).
% % \end{align*}
% % And Lemma 9.25 (ii) of \cite{kosorok2007} gives
% % \begin{align*}
% %     N_{[]}(\epsilon, \Phi_{d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}) \le N_{[]}(\epsilon / d, \Phi_{l,r,\sigma}, \|\cdot \|_{L_2(Q)})^d.
% % \end{align*}
% % Finally, by Theorem 9.24 of \cite{kosorok2007}, there exists $K$ such that
% % \begin{align*}
% %     \log N_{[]}(\epsilon / d, \Phi_{l,r,\sigma}, \|\cdot \|_{L_2(Q)}) \le d K/\epsilon,
% % \end{align*}
% % putting everything together gives
% % \begin{align*}
% %     \log N(\epsilon, \Phi_{d,l,r,\sigma}, \|\cdot \|_{L_2(Q)}) \le d^2 K/\epsilon,
% % \end{align*}
% % and writing $c_2=d^2 K$ concludes.

% Unfortunately, these numbers can't be used to bound the generalization risk, since one has to measure the complexity of the spaces of considered densities, namely
% \begin{align*}
%     \Phi_{l,r,\sigma}' &= \{g\colon g(x) = \partial_x G(x), G \in \Phi_{l,r,\sigma}\}, \\
%     \Phi_{d,l,r,\sigma}' &= \{g\colon g(x) = \partial_x G(x), G \in \Phi_{d,l,r,\sigma}\}, \\
%     \Phi_{m,d,l,r,\sigma}' &= \{g\colon g(x) = \partial_x G(x), G \in \Phi_{m,d,l,r,\sigma}\}.
% \end{align*}

% \begin{proposition}
%     Some bound on the covering numbers of $\Phi_{l,r,\sigma}'$, $\Phi_{d,l,r,\sigma}'$, and $\Phi_{m,d,l,r,\sigma}'$ (through bracketing).
% \end{proposition}

% %%%% SCRIBBLES
% %%%% SCRIBBLES
% %%%% SCRIBBLES

% % For any vector $k=(k_1, \dots, k_d)$ of $d$ integers, define the differential operator $\partial^k = \partial_{1}^{k_1} \cdots \partial_{d}^{k_d}$,
% % where $\partial_{i}^{k_i} = \partial^{k_i}/\partial_{x_i}^{k_i}$.
% % For $p \in \N \cup \{0\}$, $0 < \alpha \le 1$, 
% % and a function $f\colon \Xcal \subset \R^d \to \R$, let
% % \begin{align*}
% %     \|f\|_{p, \alpha} = \max_{k \colon \sum k_i \le p} \sup_{x \in \Xcal} |\partial^k f(x) | + \max_{k \colon \sum k_i = p } \sup_{x_1, x_2 \in \Xcal} \frac{|\partial^k f(x_1) - D^k f(x_2)|}{\| x_1 - x_2 \|^{\alpha}},
% % \end{align*}
% % and denote the H\"older space of function by $\Ccal_{\alpha, M}(\Xcal) = \{f\colon \Xcal \to \R, \|f\|_{\alpha} \le M \}$.

% % Let 
% % If $\sigma$ is sufficiently smooth, then $\log \Phi_{l,r,\sigma}'$ is $P$-GC provided that $\int |x|^{2 + \epsilon} dP(x) < \infty$  


% % \begin{align*}
% %     R(F) \le R_n(F) + \sup_{F \in \Phi_{m,d,l,r,\sigma}} |R_n(F) - R(F)|.
% % \end{align*}



% % If we can show that there exists a fixed function $G$ and a metric $d$ on $\Phi_{l,r,\sigma}$ such that
% % \begin{align*}
% %     |\log g_1(x) - \log g_2(x)| \le d(G_1, G_2) G(x), \quad \forall g_1, g_2 \in \Phi_{l,r,\sigma}',
% % \end{align*}
% % then for any norm $\| \cdot \|$
% % \begin{align*}
% %     N_{[]}(2\epsilon\|G\|,\log \Phi_{l,r,\sigma}',\| \cdot \|) \le N(\epsilon,\Phi_{l,r,\sigma},d),
% % \end{align*}
% % where $N_{[]}$ denotes the bracketing numbers.
% % Then, if one can show that $d(G_1, G_2) \le \| G_1 - G_2 \|_{L_2(Q)}$, what we need follows.

% % Alternatively, we could go the route of H\"older classes.

% % \citep[Example 2.10.8][]{vanderVaart1996} for the Donsker-preservation of the product of bounded classes


% % \subsection{Can we do more?}
% % Let $F_0 \in \Fcal_d$ be the true but unknown data-generating distribution.
% % Using the negative log-likelihood as loss function, the population risk for any $F \in \Fcal_d$ with corresponding density $f$ is $R(F) = \E_{F_0} \log f(X)$, which is uniquely minimized at $F_0$.
% % Assume that we observe an i.i.d. sample $X_1, \cdots, X_N$ with $X_i \in \R^d \sim F_0$ and that $\Fcal_{N,d} \subset \Fcal_d$, the excess risk for any estimated $\widehat{F} \in \Fcal_{N,d}$ can be decomposed as
% % \begin{align*}
% %     R(\widehat{F}) - R(F_0) = \underbrace{R(\widehat{F}) - \inf_{F \in \Fcal_{N,d}} R(F)}_{\mbox{Estimation error}} +  \underbrace{\inf_{F \in \Fcal_{N,d}}R(F) - R(F_0)}_{\mbox{Approximation error}}.
% % \end{align*}
% % First idea: use \cite{nussbaum1996} along with known results for regression using relu networks? Otherwise, \url{https://www.mdpi.com/1099-4300/21/7/627} would give consistency, but the rate would be terrible and the journal is unknown to me.
% % Questions:
% % (1) how much can I go on (e.g., 1/2 page, 1 page) ?
% % (2) can I assume that we find the ERM or should I consider the fact that we do gradient descent?
% %

==> arxiv/exp_admv.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Anomaly detection with missing values}

Let $X_1, \dots, X_N$ be an i.i.d. sample with an observation $X_j \in \R^d$ which being either \emph{normal} or an \emph{anomaly}, that is semantically distinctive but without a label to be classified as such.
Loosely speaking, an anomaly detector is a function $s \colon \R^d \to \R$ assigning an anomaly score to every value is $\R^d$.
For instance, given a density estimator $\widehat{f}$, a natural detector is $s(x) = - \log \widehat{f}(x)$ for $x\in \R^d$, that is observations with low density are potentially anomalous.

Additionally, let $M_j, \dots, M_N$ be a vector with $M_j \in \{0,1\}^d$ such that $M_{ji} = 1$ indicates that $X_{ji}$ is missing, and denote by $X_{j(0)}$ and $X_{j(1)}$ respectively the vectors of observed and missing components of $X_j$.
Assume that some values are missing at random or completely at random \citep[MAR or MCAR, see e.g., ][Section 1.3]{little2019}.
In this setup, we can ignore the missingness mechanism and the negative log-likelihood on the observed features, namely $- \sum_{j=1}^N \log f(X_{j(0)})$, is sufficient for inference.

Accounting for potential missingness, the optimal detector is then the conditional expectation of $s$ given the available information, that is
\begin{align*}
    s_{OPT}(x_{(0)}) = \int s(x) \widehat{f}(x_{(1)}|x_{(0)}) dx_{(1)}.
\end{align*}
If the integral is infeasible, an alternative is to use maximum a posteriori imputation (MAP) and compute
\begin{align*}
    s_{MAP}(x_{(0)}) = s(x_{(0)},\widehat{x}_{(1)}),\quad
    \widehat{x}_{(1)} = \mbox{argmax}_{x_{(1)}} \widehat{f}(x_{(1)}|x_{(0)}).
\end{align*}



==> arxiv/exp_toy.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Toy density estimation}
\newcommand\subfigwidth{.24\textwidth}

\begin{figure}[h]
  \centering
  \renewcommand{\tabcolsep}{1pt}
  \begin{tabular}[c]{cccc}
\begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data.pdf}
      \label{fig:caeob}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data_2d_1_2.pdf}
      \label{fig:ceoac}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data_2d_1_3.pdf}
      \label{fig:ceose}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_data_2d_2_3.pdf}
      \label{fig:ceod}
    \end{subfigure}
    \\[-.1in]
       \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_model_samples_3d.pdf}
      \label{fig:ceob}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_marg_1_2.pdf}
      \label{fig:ceoc}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_marg_1_3.pdf}
      \label{fig:ceoe}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_marg_2_3.pdf}
      \label{fig:cdfeod}
    \end{subfigure}
    \\[-.1in]
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=2.5cm, width=\textwidth]{figs/3d_spirals_1d_marg.pdf}
      \label{fig:caeob}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_cond_0.5.pdf}
      \label{fig:ceoac}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_cond_0.pdf}
      \label{fig:ceose}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[height=3cm, width=\textwidth]{figs/3d_spirals_2d_cond_-0.5.pdf}
      \label{fig:ceod}
    \end{subfigure}
  \end{tabular}    
  \caption{\textbf{Density estimation with closed-form marginals and conditionals.} \textit{Top Row:} Samples from the model after fitting a three-dimensional density, and plots of two-dimensional marginal densities learned by the model.
  \textit{Middle Row:} Samples from the training set, and marginal histograms of training data. \textit{Bottom Row:} \textit{Left:} one-dimensional marginals learned by the model compared to marginal histograms of the training data. \textit{Right:} Conditional densities learned by the model. All the marginal and conditional densities can also be sampled from efficiently (not shown).}
  \label{fig:ceo}
\end{figure}




==> arxiv/exp_toy_spirals.tex <==
%!TEX root = ../MDN_neurips.tex

\begin{figure}[h]
  \centering
  \renewcommand{\tabcolsep}{1pt}
  \begin{tikzpicture}
    \node {\begin{tabular}[c]{cccc}
\begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_data_2d_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in]
       \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_model_samples_3d.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_1_2.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_1_3.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_marg_2_3.pdf}
      \label{}
    \end{subfigure}
    \\[-.1in] % --------
    \begin{subfigure}[c]{\subfigwidth}
    \vspace{.05in}
      \includegraphics[width=\textwidth]{figs/3d_spirals_1d_marg.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_0.5.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_0.pdf}
      \label{}
    \end{subfigure}&
    \begin{subfigure}[c]{\subfigwidth}
      \includegraphics[width=\textwidth]{figs/3d_spirals_2d_cond_-0.5.pdf}
      \label{}
    \end{subfigure}
    %     \\[-.1in] % --------
    % \begin{subfigure}[c]{\subfigwidth}
    % \vspace{.05in}
    %   \includegraphics[width=\textwidth]{figs/3d_checkerboard_data.pdf}
    %   \label{}
    % \end{subfigure}&
    % \begin{subfigure}[c]{\subfigwidth}
    %   \includegraphics[width=\textwidth]{figs/3d_checkerboard_2d_marg_1_2.pdf}
    %   \label{}
    % \end{subfigure}&
    % \begin{subfigure}[c]{\subfigwidth}
    %   \includegraphics[width=\textwidth]{figs/3d_gaussians_data.pdf}
    %   \label{}
    % \end{subfigure}&
    % \begin{subfigure}[c]{\subfigwidth}
    %   \includegraphics[width=\textwidth]{figs/3d_gaussians_2d_marg_1_2.pdf}
    %   \label{}
    % \end{subfigure}
  \end{tabular}};
    % \draw[black,thick,] (-7,4.2) rectangle (7,8.3);
    %   \node[text width=3cm] at (0.6,8) 
    % {Training data};
        \draw[black,thick,] (-7,2.3) rectangle (7,6.3);
      \node[text width=3cm] at (0.6,6) 
    {Training data};
\end{tikzpicture}
  \caption{\textbf{Density estimation with closed-form marginals and conditionals.} 
  \textit{First Row:} Samples from the training set, and marginal histograms of training data.
  \textit{Second Row:} Samples from the model after fitting a three-dimensional density, \dg{clarify} and plots of two-dimensional marginal densities learned by the model.
   \textit{Third Row:} \textit{Left:} one-dimensional marginals learned by the model compared to marginal histograms of the training data. \textit{Right:} Conditional densities learned by the model. All the marginal and conditional densities can also be sampled from efficiently.
  \textit{Fourth Row:} Results on additional datasets: \textit{Left:} Training data and learned marginal density for a 3D checkerboard dataset. \textit{Right:} Training data and learned marginal density for a 3D mixture of Gaussians.
   }
  \label{fig:2spirals}
\end{figure}

==> arxiv/mdma.tex <==
%!TEX root = ../MDN_neurips.tex

\section{Marginalizable Density Models}
\label{sec:marginalizable_models}

\subsection{Notation}
In the following, we use a capital and lowercase Roman letter (e.g., $F$ and $f$) or Greek letters along with dot above (e.g., $\varphi$ and $\varphid$) to denote respectively absolutely continuous CDFs of arbitrary dimensions and the corresponding densities. When dealing with multivariate distributions, the marginal or conditional distribution over a subset of variables will be indicated by the argument names (i.e. $F(x_{1}|x_{2},x_{3})=\mathbb{P}\left[X_{1}\leq x_{1}|X_{2}=x_{2},X_{3}=x_{3}\right]$).

For a positive integer $p \in \N \setminus 0$, 
let $[p] = \{1, \dots, p\}$.
% If $S$ is a set, then $|S|$ and $S^{\times p}$ denote respectively its cardinality and the product set $S \times \cdots \times S$ with $|S^{\times p}| = |S|^p$.
Denote the space of absolutely continuous univariate and $d$-dimensional CDFs respectively by $\Fcal_1$ and $\Fcal_d$. 
% \begin{align*}
%      \Fcal_1 &= \{F \colon \R \to [0,1],\, \lim_{x \to -\infty} F(x) = 0,\, \lim_{x \to \infty} F(x) = 1,\, \partial F(x)/\partial x \ge 0 \},\\
%     \Fcal_d &= \{F \colon \R^d \to [0,1],\, \lim_{x_j \to -\infty} F(x_1, \dots, x_j, \dots, x_d) = 0\,\, \forall j \in [d],\, \lim_{x \to \infty} F(x, \dots, x) = 1, \\
%     &\phantom{\Fcal_d = \{F \colon \R^d \to [0,1]}\partial^{|k|} F(x_{1}, \dots, x_{d}) /\partial x_{i_{1}} \cdots \partial x_{i_{|k|}} \ge 0\,\, \forall k \subseteq [d]\}.
% \end{align*}
For any $F \in \Fcal_1$, the density $f:\R \to \R_{+}$ is $f(x) = \partial F(x)/\partial x$.
Similarly, for any $F \in \Fcal_d$, the density $f(\bm x):\R^d \to \R_{+}$ is $f(\bm x) = \partial^d F(\bm x)/\partial x_1 \cdots \partial x_d$,
and $F_j(x) = \lim_{z \to \infty} F(z, \dots, x, \dots, z) \in \Fcal_1$ for $j \in [d]$ is the $j$th marginal distribution.
% For an order $d$ tensor $A \in \R^{m_1 \times \cdots m_d}$, we use $\|A\|_1$ to denote the ``entrywise'' 1-norm, that is
% \begin{align*}
%     \|A\|_1 =\sum\limits_{i_1=1}^{m_1} \cdots \sum\limits_{i_d=1}^{m_d} |A_{i_1, \dots, i_d}|.
% \end{align*}

\subsection{The bivariate case}
For the task of modeling joint distributions of two variables supported on $\mathbb{R}^{2}$,
consider a family of univariate CDFs
$\{\varphi_{i,j}\,\}_{i\in[m],\,j\in[2]}$ with $\varphi_{i,j} \in \Fcal_1$, i.e., the functions 
$\varphi_{i,j}:\mathbb{R} \rightarrow [0,1]$ satisfy
\begin{align}
\varphi_{i,j}(-\infty) = 0 \,, \qquad     
\varphi_{i,j}(+\infty) = 1 \,, \qquad     
\dot{\varphi}_{i,j}(x_{j})  \geq 0 \,.
\end{align}
These functions will be our basic building block, 
and we model them using a simple neural architecture proposed in~\cite{balle2018variational}, which we review in~\Cref{app:univariate_marginal_param}. 
If $A$ is an $m \times m$ matrix of nonnegative elements satisfying $\sum_{i,j=1}^m A_{i,j} =1$,
we can combine it with the univariate CDFs to obtain
\begin{align} 
\label{eq:bivariate_cdf}
    F(x_{1},x_{2})=\sum\limits_{i,j=1}^{m} A_{i,j}\varphi_{i,1}(x_{1})\varphi_{j,2}(x_{2}).
\end{align}
The coefficients $A_{i,j}$ encode the dependencies between the two variables, and the normalization ensures that $F$ is a valid CDF, that is $F \in \Fcal_2$.
Even though in each summand the interaction is modeled by a single scalar parameter, such a model can be used to approximate well complex interactions between $x_1$ and $x_2$ if $m$ is sufficiently large, as we show in \Cref{sec:theory}. 
The advantage of this construction is that $\{\varphid_{i,j}\}_{i\in[m],\,j\in[2]}$, the family of densities corresponding to the univariate CDFs, leads immediately to 
\begin{align*}
f(x_{1},x_{2})=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2}). 
% f(x_{1},x_{2})=\partial^{2}F(x_{1},x_{2})/\partial x_{1}\partial x_{2}=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2}). 
\end{align*}
It is similarly straightforward to obtain marginal and conditional quantities, e.g.:
\begin{align*}
F(x_{1})&=\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1}), 
\qquad &f(x_{1})&=\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1}),  \\
    F(x_{1}|x_{2})&=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})}, 
\qquad &f(x_{1}|x_{2})&=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})}.
    % F(x_{1})&=\lim_{x_2 \to \infty }F(x_{1},x_2)=\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1}), \\
    % F(x_{1}|x_{2})&=\frac{\partial F(x_{1},x_{2})/\partial x_{2}}{\partial F(x_{2}) /\partial x_{2}}=\frac{\sum\limits_{i,j=1}^{m}A_{i,j}\varphi_{i,1}(x_{1})\varphid_{j,2}(x_{2})}{\sum\limits_{i,j=1}^{m}A_{i,j}\varphid_{j,2}(x_{2})},
\end{align*}
Deriving these simple expressions 
relies on the fact that \eqref{eq:bivariate_cdf} combines the univariate CDFs linearly. Nonetheless, it is clear that, with $m \to \infty$ and for judiciously chosen univariate CDFs, such a model is a universal approximator of both CDFs and sufficiently smooth densities.

% And since evaluating the density requires taking derivatives with respect to all inputs, fully general nonlinear models can lead to a space and time complexity that is exponential in the number of variables.
% There is thus a tension between the ability to expressively model dependencies and obtain closed-form expressions for the density as well as all marginal and conditional quantities.


\subsection{The multivariate case}\label{sec:multivariate}

% \begin{figure}
%     \centering
%     \includegraphics[height=2in]{figs/tensors.jpg}
%     \caption{\textbf{Tensor decompositions}. a) Notation for tensors of various order (vectors, matrices, delta tensors). Each edge represents an index, and connecting two edges represents contraction (summation over an index). b) A general unstructured tensor of order d. c) The set of univariate CDFs. d)  
%     The CP decomposition and the hierarchical Tucker (HT) decomposition.}
%     \label{fig:tensor_decomps}
% \end{figure}

% Extending the above construction to the multivariate case, we are thus confronted with the problem of combining products of univariate CDFs linearly, in a manner that is both computationally efficient and expressive. %A sum over all possible products for example will require $n^d$ parameters and is thus impractical even for moderate $d$. 
% The linearity constraint reduces this to a tensor decomposition problem (with additional non-negativity and normalization constraints). There is an extensive literature on such efficient tensor decompositions (see \cite{Cichocki2017-gp} for a review). A graphical representation of the tensor decompositions used in this work is presented in \Cref{app:tensor_decomps}. %For example, a fundamental problem in many-body quantum mechanics is the efficient representation of the state of a many-body system, which is in fact a multivariate distribution, in terms of states of single particles defined in terms of univariate distributions. (add more examples?). 

% The analogy with tensor decompositions becomes clear when we consider discrete rather than continuous variables.
% Say we wish to model the joint distribution of $d$ discrete variables, each taking one of $S$ possible values.
% The distribution is then a function $\varphi_{S}:[S] \times \cdots \times [S] \rightarrow\mathbb{R}$, which can also be viewed as an order $d$ tensor.
% %We can represent tensors of any order graphically using standard notation in \cref{fig:tensor_decomps}a.
% A general tensor $\varphi_{S}$ %(as in the left of \cref{fig:tensor_decomps}b) 
% will require order of $S^d$ numbers to represent, and is thus impractical even for moderate $d$.
% The continuous analog of such a tensor is a multivariate function $F:\mathbb{R}^{d}\rightarrow\mathbb{R}$, with the value of $x_j$ corresponding to the discrete index $s_j$.
% We will thus use the same notation for the continuous case. 

To generalize the bivariate case, consider a collection of univariate CDFs $\{\varphi_{i,j}\}_{i\in[m],\,j\in[d]}$ with $\varphi_{i,j} \in \Fcal_1$ for each $i$ and $j$, and define the tensor-valued function $\Phi \colon \R^d \to [0,1]^m \times \cdots \times [0,1]^m$ by $\Phi(\bm x)_{i_1, \dots, i_d} = \prod_{j=1}^{d}\varphi_{i_{j},j}(x_{j})$ for $\bm x \in \R^d$.
Furthermore, denote the class of normalized order $d$ tensors with $m$ dimensions in each mode and nonnegative elements by
\begin{align}
    \Acal_{d,m} = \{A \in \R^{m \times \cdots \times m}\colon A_{i_1, \dots, i_d} \ge 0,\, \sum\limits_{i_1, \dots, i_d = 1}^m A_{i_1, \dots, i_d} = 1 \}.
    \label{eq:define_acal}
\end{align}
\begin{definition}[Marginalizable Distribution Model Approximator]
For $\Phi \colon \R^d \to [0,1]^m \times \cdots \times [0,1]^m$ as above and $A \in \Acal_{d,m}$,
the marginalizable distribution model approximator (MDMA) is
\begin{align} \label{eq:F_general_A}
    F_{A,\Phi}(\bm x)= \langle A, \Phi(\bm x) \rangle  = \sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\prod\limits_{j=1}^{d}\varphi_{i_{j},j}(x_{j}).
\end{align}
\end{definition}
If is clear that the conditions on $\Phi$ and $A$ imply that $F_{A,\Phi} \in \Fcal_d$.  
As in the bivariate case, densities or marginalization over $x_j$ are obtained by replacing each $\varphi_{i,j}$ respectively by $\varphid_{i,j}$ or $1$. 
As for conditioning, considering any disjoint subsets $R=\left\{ k_{1},\dots,k_{r}\right\}$ and $S=\left\{ j_{1},\dots,j_{s}\right\}$ of $[d]$ such that $R \cap S = \emptyset $, we have  
\begin{align*}
F_{A, \Phi}(x_{k_{1}},\dots,x_{k_{r}}|x_{j_{1}},\dots,x_{j_{s}}) & = \frac{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{k\in R}{\prod}\varphi_{i_{k},k}(x_{k})\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}.
%  f(x_{k_{1}},\dots,x_{k_{r}}|x_{j_{1}},\dots,x_{j_{s}}) &= \frac{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{k\in R}{\prod}\varphid_{i_{k}k}(x_{k})\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}{\sum\limits_{i_{1},\dots,i_{d}=1}^{m}A_{i_{1},\dots,i_{d}}\underset{j\in S}{\prod}\varphid_{i_{j},j}(x_{j})}.
\end{align*}
% and similarly the conditional density is obtained by replacing $\varphi_{i_{k},k}(x_{k})$ by $\varphid_{i_{k},k}(x_{k})$.

For a completely general tensor $A$, the expression \eqref{eq:F_general_A} is computationally impractical since such a model has $O(m^d)$ parameters, hence some structure must be imposed on $A$.
For instance, using $A_{i_1, \dots, i_d}=a_{i_1} \delta_{i_1, \dots, i_d}$ leads to $F_{A,\Phi}(\bm x)=\sum_{i=1}^m a_{i}\prod_{j=1}^{d}\varphi_{i,j}(x_{j})$, with $a_i \ge 0$ and $\sum_{i=1}^m a_{i} = 1$.
Instead this top-down approach, $A$ can be tractably constructed bottom-up, as we explain next. 
% A natural choice is the so-called order $m$ CP decomposition, given by
% \begin{align}\label{eq:CP}
%     F_{\mathrm{CP}}(x_{1},\dots,x_{d})=\sum\limits_{i=1}^m a_{i}\prod\limits_{j=1}^{d}\varphi_{i,j}(x_{j}),
% \end{align}
% where $a$ is an $m \times 1$ vector with nonnegative elements such that $\sum_{i=1}^m a_i=1$.
% This is clearly a valid CDF and can be made more expressive by increasing $m$. 
% A more powerful parametrization of $A$ is a variant of the hierarchical Tucker (HT) decomposition first introduced in \cite{Hackbusch2009-yr}%, which we illustrate in \Cref{fig:tensor_decomps}e.
% Such tensors were used in the construction of deep linear convolutional networks for image classification in \cite{cohen2016expressive}.
% Specifically, we take the coefficients in \cite{Hackbusch2009-yr} to be diagonal with respect to their lower indices and fix the pool size as 2, yet for brevity refer to such a decomposition henceforth as the HT decomposition.
% Fixing a pool size 2 and 

Assuming for simplicity that $d$ is an integer power of 2, let $\varphi^{1} \colon \R^d \to \R^{m \times d}$ be the matrix-valued function defined by $\varphi^{1}_{i,j}(\bm x) = \varphi_{i,j}(x_j)$.
For $l \in \{2, \dots, \log_2 d\}$, define the matrix-value functions $\varphi^{l}\colon \R^d \to \R^{m \times d/2^{l-1}}$ recursively by 
\begin{align}\label{eq:HT_recurs}
\varphi_{i,j}^{l}(\bm{x})=\sum\limits _{k=1}^{m}\lambda_{i,k,j}^{l-1}\varphi_{k,2j-1}^{l-1}(\bm{x})\varphi_{k,2j}^{l-1}(\bm{x}),
\end{align}
where $\lambda^{l}$ is an $m \times m \times d/2^{l}$ tensor.
The CDF can then be written as
\begin{align} \label{eq:HT}
 F_{A, \Phi}(\bm x) &= \sum\limits_{k=1}^m a_{k} \varphi_{k,1}^{\log_{2}d}(\bm x)\varphi_{k,2}^{\log_{2}d}(\bm x),
\end{align}
with $a \in \mathbb{R}^m$. %an $m \times 1$ vector as in \eqref{eq:CP}.
If all parameters are nonnegative, $\sum_{k=1}^m \lambda_{i,k,j}^{l}=1$ for all $l$, and $\sum_{k=1}^m a_k=1$, it is easy to verify that the underlying $A$ satisfies $A \in \Acal_{d,m}$ defined in (\ref{eq:define_acal}). 
As a concrete example, for $d=4$, we have 
\begin{align*}
% F_{\mathrm{HT}}(\bm x)  
%   &= \sum\limits_{k_1,k_2,k_2'=1}^m a_{k_1} \lambda_{k_2,k_1,1}^{1}\lambda_{k_2',k_1,2}^{1}\varphi_{k_2,1}^{1}(\bm x)\varphi_{k_2,2}^{1}(\bm x)\varphi_{k_2',3}^{1}(\bm x)\varphi_{k_2',4}^{1}(\bm x) 
F_{A, \Phi}(\bm{x})=\sum\limits _{k_{2},k_{1},k_{1}'=1}^{m}a_{k_{2}}\lambda_{k_{2},k_{1},1}^{1}\lambda_{k_{2},k_{1}',2}^{1}\varphi_{k_{1},1}^{1}(\bm{x})\varphi_{k_{1},2}^{1}(\bm{x})\varphi_{k_{1}',3}^{1}(\bm{x})\varphi_{k_{1}',4}^{1}(\bm{x})
\end{align*}
from which we can read off that $A_{i_{1},i_{2},i_{3},i_{4}}=\sum_{k=1}^{m}a_{k}\lambda_{k,i_{1},1}^{1}\lambda_{k,i_{3},2}^{1}\delta_{i_{1},i_{2}}\delta_{i_{3},i_{4}}$. Note that the number of parameters required to represent $A$ is only $\mathrm{poly}(m,d)$.
The construction can be generalized straightforwardly to cases where $d$ is not divisible by 2, and/or the pool size is any positive integer.
It is in fact a variant of the hierarchical Tucker decomposition \cite{Hackbusch2009-yr}, which has been used in the construction of tensor networks for image classification in \cite{cohen2016expressive}.  
A graphical representation of this tensor is provided in \Cref{fig:tensor_decomps} in the supplementary materials.  
We present additional details regarding the choice of architecture and initialization in \Cref{app:design_details}. 

\subsection{A non-marginalizable variant} \label{sec:nmdma}

We can construct a more expressive variant of MDMA at the price of losing the ability to marginalize and condition on arbitrary subsets of variables. We find that the resulting model leads to state-of-the-art performance on a density estimation benchmark.
We define $\mathbf{v}=\mathbf{x}+\mathbf{T}\sigma(\mathbf{x})$ where $\mathbf{T}$ is an upper-triangular matrix with non-negative entries and $0$ on the main diagonal. Note that $\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}}\right|=1$.
Given some density $f(v_{1},\dots,v_{d})=\prod\limits_{j=1}^{d}\varphid_{j}(v_{j})$, we have 
\begin{align}
f(x_{1},\dots,x_{d})=\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}}\right|f(v_{1},\dots,v_{d})=f(v_{1}(\mathbf{x}),\dots,v_{d}(\mathbf{x})).
\end{align}
We refer to this model nMDMA, since it is \textit{non}-marginalizable.  
% {\color{red}
% It follows that 
% \eqan
% F(x_{1},\dots,x_{d})&=&\int_{-\infty}^{\mathbf{x}}\prod\limits_{j=1}^{d}dx_{j}'f(x'_{1},\dots,x'_{d})\\
% &=&\int_{-\infty}^{\mathbf{x}}\prod\limits_{j=1}^{d}dx'_{j}\left|\frac{\partial\mathbf{v}}{\partial\mathbf{x}'}\right|f(v_{1}(\mathbf{x}'),\dots,v_{d}(\mathbf{x}'))\\
% &=&\int_{-\infty}^{\mathbf{v}(\mathbf{x})}\prod\limits_{j=1}^{d}dv'_{j}f(v'_{1},\dots,v'_{d})\\
% &=&\prod\limits_{j=1}^{d}\varphi_{j}(v_{j}(\mathbf{x})).
% \enan
% Marginalizing over a subset of the $x_j$ is done by setting these variables to $\infty$ in the expression $\underset{j=1}{\overset{d}{\Pi}}\varphi_{j}(v_{j}(\mathbf{x}))$. The marginal density can be obtained by taking derivatives of the marginal CDF. For a block-triangular matrix with block size $S$ this will generate no more than $Sd$ terms. Conditional PDFs and CDFs can be obtained from the marginals and the joints as before. 

% We can also include permutations to group the variables in different ways. 
% % In order to combine this approach with the HT decomposition of the tensor $A$, we simply set the permutation matrix $P$ to be an identity. This ensures that each summand in the expression $\left\langle A,\Phi(\mathbf{y})\right\rangle $ is a valid CDF.  
% }
% \subsection{A simple example}
% Consider the transformation 
% \eqan 
% v_1 &=& x_1
% \\
% v_2 &=& \alpha \sigma(x_1) + x_2
% \enan 
% We model the CDF of $(v_1,v_2)$ as
% \eqan 
% F(v_1,v_2) = \phi_{1}(v_1) \phi_2(v_2)
% \label{eq:CD\varphi_v}
% \enan
% and the pdfs is
% \eqan 
% p(x_1,x_2) &=& p(v_1,v_2) 
% \\
% &=&  \phi_{1}'(v_1) \phi_2'(v_2)
% \\
% &=& \phi_{1}'(x_1) \phi_2'(\alpha \sigma(x_1) + x_2)
% \label{eq:density_v}
% \enan 
% where we used that the 
% Jacobian is unity. 

% To obtain the marginal $p(x_2)$, we start 
% with the CFD
% \eqan 
% F(x_2, x_1=\infty) = \phi_2(\alpha +x_2),
% \enan 
% where we used (\ref{eq:CD\varphi_v}), 
% and take the derivative w.r.t. $x_2$,
% \eqan 
% p(x_2) = \phi_2'(\alpha +x_2)\,.
% \enan 
% To verify that this expression is consistent with (\ref{eq:density_v}), note that 
% \eqan 
% \int_{-\infty}^{+\infty}dx'_1 p(x'_1,x_2) &=& \int_{-\infty}^{+\infty}dx'_1\phi_{1}'(x'_1) \phi_2'(\alpha \sigma(x'_1) + x_2)
% \\
% &=& \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{+\infty}dx'_1
% \int_{-\infty}^{+x_2}dx'_2
% \phi_{1}'(x'_1) 
% \phi_2'(\alpha \sigma(x'_1) + x_2')
% \\
% &=&
% \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{+\infty}dv'_1
% \int_{-\infty}^{\alpha +x_2  }dv'_2
% \phi_{1}'(v'_1) 
% \phi_2'(v_2')
% \\
% &=&
% \int_{-\infty}^{+\infty}dv'_1
% \phi_{1}'(v'_1) 
% \, \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \\
% &=& \phi_2'(\alpha + x_2)
% \enan 

% \subsubsection*{Three variables}
% \eqan 
% p(x_1,x_2,x_3) &=& p(v_1,v_2,v_3) 
% \\
% &=&  \phi_{1}'(v_1) \phi_2'(v_2) \phi_3'(v_3)
% \\
% &=& \phi_{1}'(x_1) \phi_2'(\alpha \sigma(x_1) + x_2)
% \phi_3'(\alpha_{31} \sigma(x_1) + \alpha_{32} \sigma(x_2) + x_3)
% \label{eq:density_v3}
% \enan 
% where we used that the 
% Jacobian is unity. 

% % To obtain the marginal $p(x_2,x_3)$, we start 
% % with the CFD
% % \eqan 
% % F(x_2, x_1=\infty) = \phi_2(\alpha +x_2),
% % \enan 
% % where we used (\ref{eq:CD\varphi_v}), 
% % and take the derivative w.r.t. $x_2$,
% % \eqan 
% % p(x_2) = \phi_2'(\alpha +x_2)\,.
% % \enan 
% % To verify that this expression is consistent with (\ref{eq:density_v}), note that 
% {\tiny 
% \eqan 
% \int_{-\infty}^{+\infty}dx'_1 p(x'_1,x_2,x_3) &=&
% \int_{-\infty}^{+\infty}dx'_1
% \phi_{1}'(x_1') \phi_2'(\alpha \sigma(x_1') + x_2)
% \phi_3'(\alpha_{31} \sigma(x_1') + \alpha_{32} \sigma(x_2) + x_3)
% \nn 
% \\
% &=& \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{+\infty}dx'_1
% \int_{-\infty}^{+x_2}dx'_2
% \int_{-\infty}^{+x_3}dx'_3
% \phi_{1}'(x_1') \phi_2'(\alpha \sigma(x_1') + x_2')
% \phi_3'(\alpha_{31} \sigma(x_1') + \alpha_{32} \sigma(x_2') + x_3')
% \nn 
% \\
% &=&
% \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{+\infty}dv'_1
% \int_{-\infty}^{\alpha +x_2  }dv'_2
% \int_{-\infty}^{\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3 }dv'_3
% \phi_{1}'(v'_1) 
% \phi_2'(v_2')
% \phi_3'(v_3')
% \\
% &=&
% \int_{-\infty}^{+\infty}dv'_1
% \phi_{1}'(v'_1) 
% \, 
% \frac{\partial^2}{\partial x_2 \partial x_3} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \int_{-\infty}^{\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3 }dv'_3 \phi_3'(v_3')
% \\
% &=& 
% \frac{\partial}{\partial x_2} 
% \int_{-\infty}^{\alpha + x_2}dv'_2
% \phi_2'(v_2')
% \phi_3'(\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3)
% \\
% &=& 
% \frac{\partial}{\partial x_2} 
% \left[ 
% \phi_2(\alpha + x_2)
% \phi_3'(\alpha_{31} + \alpha_{32} \sigma(x_2)  + x_3)
% \right]
% \enan 
% }


\subsection{Efficient sampling}
{\color{red}TODO: update notation}

{\color{red}can drop this paragraph}
Given a model of a multivariate CDF \cref{eq:F_general_A} we can readily compute the conditional univariate CDFs and invert them numerically, which allows for sampling in the same manner as other autoregressive models.
To be precise, sampling a vector $(u_{1},\dots,u_{d})$ of independent components from the uniform distribution, we obtain a sample from $F$ by computing 
\begin{equation}
x_{1} =F_{A,\Phi}^{-1}(u_{1}),\quad x_{i} = F_{A,\Phi}^{-1}(u_{i}|x_{1},\dots,x_{i-1}),
\end{equation}
(where unlike other autoregressive model, the order of taking the conditionals need not be fixed).
The main drawback of this method is that due to the sequential nature of the sampling the computational cost is linear in $d$ and cannot be parallelized.
In addition, evaluation of the inverse conditional CDFs requires evaluating multiple forward passes of the model. 

However, the structure of $F_{A,\Phi}$ defined in \cref{eq:F_general_A} can be leveraged to sample much more efficiently.
Define by $R_{A}$ a vector-valued categorical random variable taking values in $\left[m\right]^{\times d}$, with distribution 
\begin{equation}
    \mathbb{P}\left[R_{A}=(i_{1},\dots,i_{d})\right]=A_{i_{1},\dots,i_{d}}.
\end{equation}
The fact that $A$ is nonnegative and satisfies $\|A\|_1=1$ ensure the validity of this definition.
Consider a vector $(\tilde{X}_{1},\dots,\tilde{X}_{d},R_{A})$ where $R_A$ is distributed as above, and 
\begin{equation}
    \mathbb{P}\left[\tilde{X}_{1}\leq x_{1},\dots,\tilde{X}_{d}\leq x_{d}|R_{A}=\mathbf{r}\right]=\prod\limits_{i=1}^{d}\varphi_{r_{i},i}(x_{i}),
\end{equation}
for a collection $\{\varphi_{i,j}\}$ of univariate CDFs. Denoting the distribution of this vector by $\tilde{F}_{A,\Phi}$, marginalizing over $R_A$ gives 
\begin{equation}
	\tilde{F}_{A,\Phi}(x_{1},\dots,x_{d})=\underset{\mathbf{r}\in[m]^{d}}{\sum}\mathbb{P}\left[R_{A}=\mathbf{r}\right]\prod\limits_{j=1}^{d}\varphi_{r_{j},j}(x_{j})
	%=\underset{i_{1},\dots,i_{d}=1}{\overset{m}{\sum}}A_{i_{1},\dots,i_{d}}\prod\limits_{i=1}^{d}\varphi_{i_{j},j}(x_{j})
	=F_{A,\Phi}(x_{1},\dots,x_{d}).
\end{equation}
Instead of sampling directly from the distribution $F_{A,\Phi}$, we can thus sample from $\tilde{F}_{A,\Phi}(x_{1},\dots,x_{d})$ and discard the sample of $R_A$. To do this, we first sample from the categorical variable $R_A$. Denoting this sample by $\mathbf{r}$, we can sample from $\tilde{X}_{i}$ by inverting the univariate CDF $\varphi_{r_{i},i}$. This can be done \textit{in parallel} for all $i$. 

The approach outlined above is impractical since $R_{A}$ can take $m^d$ possible values, yet if $A$ can be expressed by an efficient tensor representation this exponential dependence can be avoided. Consider the HT decomposition \cref{eq:HT}. It can be written as 
\begin{equation}
\left\langle A,\Phi\right\rangle =\underset{\ell,j_{\ell}}{\prod}\underset{k_{\ell,j_{\ell}}=1}{\overset{m_{\ell}}{\sum}}a_{k_{\ell-1,\left\lceil j_{\ell}/2\right\rceil },j_{\ell}}^{\ell,k_{\ell,j_{\ell}}}\Phi_{k_{1,1},\dots,k_{1,\left\lceil d/2\right\rceil }}.
\end{equation}
%which is a normalized sum of $O(md)$ CDFs. We can sample from this mixture in $O(\log d)$ time and requiring the storage of only $O(d)$ integers. 

Define a collection of independent categorical variables $\{R^\ell_{i,j}\}$ taking values in $[m_\ell]$, such that 
\begin{equation}
	\forall\ell,i,j:\quad\mathbb{P}\left[R_{i,j}^{\ell}=k\right]=a_{i,j}^{\ell,k},
\end{equation}
where $\left\{ a_{i,j}^{\ell,k}\right\}$ are the parameters of the HT decomposition (our normalization of the HT coefficients ensures that this is a valid distribution).

If we define a random vector $(\tilde{X}_{1},\dots,\tilde{X}_{d})$ as before such that
\begin{equation}
\mathbb{P}\left[\tilde{X}_{1}\leq x_{1},\dots,\tilde{X}_{d}\leq x_{d}|R^{1}=\mathbf{k}_{1}\cap R^{2}=\mathbf{k}_{2}\cap\dots\cap R^{\ell_{d}}=k_{\ell_{d}}\right]=\prod\limits _{i=1}^{d}\varphi_{k_{1,i/2},i}(x_{i}),
\end{equation}
 we again find that the distribution of $(\tilde{X}_{1},\dots,\tilde{X}_{d})$ obtained by marginalizing over $\{R^\ell_{i,j}\}$ is equal to $F_{\mathrm{HT}}$, hence we can sample from $(\tilde{X}_{1},\dots,\tilde{X}_{d},\{R_{i,j}^{\ell}\})$ instead.

Sampling $\{R_{i,j}^{\ell}\}$ is best done sequentially starting from the final layer. We first sample from $R^{\ell_d}$ obtaining a sample $k_{\ell_d}$. We next sample from $R_{k_{\ell_{d}},1}^{\ell_{d}-1},R_{k_{\ell_{d}},2}^{\ell_{d}-1}$ obtaining samples $k_{\ell_{d}-1,1},k_{\ell_{d}-1,2}$ and proceed similarly until the reaching the first layer. There are $\left\lceil \log_2 d\right\rceil $ layers in the decomposition, and aside from storing the decomposition itself this sampling procedure requires storing only $O(d)$ integers. Since 
\begin{equation}
	\mathbb{P}\left[R^{\ell_{d}}=k_{\ell_{d}}\cap R_{k_{\ell_{d}},1}^{\ell_{d}-1}=k_{\ell_{d}-1,1}\cap R_{k_{\ell_{d}},2}^{\ell_{d}-1}=k_{\ell_{d}-1,2},\dots,R_{k_{2,d/2},d/2}^{1}=k_{1,d/2}\right]=\underset{\ell,j_{\ell}}{\prod}a_{k_{\ell-1,\left\lceil j_{\ell}/2\right\rceil },j_{\ell}}^{\ell,k_{\ell,j_{\ell}}},
\end{equation}
sampling from the categorical variables in this fashion is equivalent to sampling a mixture component. We then sample $\tilde{X}_{i}$ by inverting the univariate CDF $\varphi_{k_{1,\left\lceil i/2\right\rceil },i}(x_{i})$, parallelizing over $i$. Note that the time complexity of this sampling depends only logarithmically on $d$, and this logarithmic dependence is only in the sampling from the categorical variables which is inexpensive to begin with. We thus avoid the linear dependence on $d$ that is common in sampling from autoregressive models. 


==> arxiv/sampling.tex <==
%!TEX root = ../MDN_neurips.tex

\subsection{Sampling}
\begin{align*}
\begin{aligned}
    k_p & \sim \textrm{Mult}(\lambda_{*}^p)
    \\
    k_{p-1,j} & \sim \textrm{Mult}(\lambda^{p-1}_{k_p, *,j}) & j=1,2
    \\
    k_{p-2,j} & \sim \textrm{Mult}(\lambda^{p-2}_{k_{p-1, j/2  }, *,j}) & j=1,2,3,4
    \\
    \vdots
    \\
    k_{1,j} & \sim \textrm{Mult}(\lambda^{1}_{k_{2,  j/2  }, *,j}) & j=1 \ldots 2^{p-1}
    \\
    x_j & \sim \varphi_{k_{1, j/2   },j}(x_j)  & j=1 \ldots 2^{p}
\end{aligned}
\end{align*}
